A Polynomial-time, Truthful, Individually Rational and Budget Balanced Ridesharing Mechanism

Ridesharing has great potential to improve transportation efficiency while reducing congestion and pollution. To realize this potential, mechanisms are needed that allocate vehicles optimally and provide the right incentives to riders. However, many existing approaches consider restricted settings (e.g., only one rider per vehicle or a common origin for all riders). Moreover, naive applications of standard approaches, such as the Vickrey-Clarke-Groves or greedy mechanisms, cannot achieve a polynomial-time, truthful, individually rational and budget balanced mechanism. To address this, we formulate a general ridesharing problem and apply mechanism design to develop a novel mechanism which satisfies all four properties and whose social cost is within 8.6% of the optimal on average.

==> SOTON IJCAI2021/arxivfooter.tex <==
\thispagestyle{fancy}
\pagestyle{fancy}
\fancyhf{}
\renewcommand{\headrulewidth}{0pt}
\lfoot[Copyright International
Joint Conferences on Artificial Intelligence (\href{https://ijcai.org}{IJCAI}), 2021. All rights
reserved.]{Copyright International
Joint Conferences on Artificial Intelligence (\href{https://ijcai.org}{\urlblue{IJCAI}}), 2021. All rights
reserved.}



==> SOTON IJCAI2021/cameraready.tex <==
\begin{abstract}
Ridesharing has great potential to improve transportation efficiency while reducing congestion and pollution. To realize this potential, mechanisms are needed that allocate vehicles optimally and provide the right incentives to riders. However, many existing approaches consider restricted settings (e.g., 
only one rider per vehicle
or a common origin for all riders). Moreover, 
naive applications of standard approaches, such as the Vickrey-Clarke-Groves or greedy mechanisms, cannot achieve a polynomial-time, truthful, individually rational and budget balanced mechanism. To address this, we formulate a general ridesharing problem and apply mechanism design to develop a novel mechanism which satisfies all four properties and whose social cost is within 8.6\% of the optimal on average.
\if\arxiv0
\renewcommand{\thefootnote}{}
\footnote[0]{\camera{An extended version including technical appendices is available at \href{https://arxiv.org/abs/2105.11292}{https://arxiv.org/abs/2105.11292}.}}
\renewcommand{\thefootnote}{\arabic{footnote}}
\fi
\end{abstract}

\setcounter{section}{0}

\section{Introduction}
\label{sec:intro}

Ridesharing can meet more traffic demand with fewer vehicles than existing taxi services or privately-owned vehicles. At the same time, it can reduce traffic congestion, energy consumption and pollution. Moreover, with the introduction of autonomous vehicles, unused vehicles become active transportation resources, and ridesharing can further increase utilization of such vehicles
%Studies show it is possible to reduce the number of vehicles by a third when combining the two 
\cite{Spieser2014}. 
%\modified{It also provides a way to design more dynamic and flexible public transportation options that do not need to rely on fixed routes and timetables.} 

Broadly, there are two research streams addressing ridesharing problems: \modified{the first }one focuses on algorithms for assigning vehicles to riders while solving the routing problem in an optimal way \cite{Laporte2007,Hasan2018,Chen2019}.
%; and one that focuses on the incentives and payments using mechanism design. 
%In terms of the former, early work on specific algorithms includes the Dial-a-Ride Problem (DARP) \cite{Laporte2007}, 
%\cite{Laporte2007,Agatz2012}, 
%which can be formulated as an integer linear program (ILP). Other studies formulate the ridesharing problem as a mixed integer program (MIP) \cite{Ghosh2016,BistaffaFilippo2018,Hasan2018}. To deal with the computational complexity, some studies consider the problem at a higher level and omit the computation of the routing \cite{DickersonJohnP.2018,Chen2019}.
%Yet other studies restrict the set of feasible solutions using knowledge of proximity among vehicles and riders, thereby reducing the search space \cite{Biswas,Pelzer2015,Bistaffa2015}. These studies only consider settings where riders can use a single vehicle to complete the journey.
However, none of these studies consider incentives and whether it is in the best interest of riders to follow the proposed solution and to report their preferences truthfully. Especially when the origins and  destinations of the riders are different, they are sometimes required to detour to share the vehicle with others. Hence, there may be an incentive to misreport time constraints and preferences to prevent detours.

\color{\newcolor}
To address this, the second research stream focuses on mechanism design approaches, which incentivize truthful reporting and  avoid strategic manipulation. In addition to this property, which is called incentive compatibility (IC), other desirable properties include (weak) budget balance (BB, i.e., the system does not require an outside subsidy),  individual rationality (IR, i.e., an individual is never worse off participating in the mechanism) and scalability (i.e., the allocation and any payments can be computed in polynomial time). %Moreover, we focus on settings that are capable both manual and autonomous vehicles. 
%Mechanism design for ridesharing is still largely an open problem. 
An early approach uses a second price auction \cite{Kleiner}, but their work is limited to single riders per vehicle and does not allow  cooperation between drivers. \cite{Crandall2001}  propose an online posted-price mechanism but they only consider autonomous vehicles (vehicles can move without any riders allocated) and their approach is not scalable. Furthermore, \cite{Cheng2014} propose a mechanism that satisfies IC, BB and IR, but they assume all riders depart from the same origin and so their method does not coordinate the pickup of riders at different locations. \cite{Zhao} propose a Vickrey–Clarke–Groves (VCG) mechanism, but their approach is not scalable and BB is only satisfied when there is no detour. More recent work on mechanism design, e.g., \cite{Rheingans-yoo2019,LuAlicePeterI.Frazier2018,MaHongyaoFeiFang2019}, only focuses on drivers and does not consider rider incentives. Also, none of the above consider settings where riders can switch vehicles which can enable more efficient solutions, especially in settings with limited vehicles as in suburban areas. 
%Though mechanism design has been applied to ridesharing problems, there are issues that
%\cite{Kleiner} propose a second price auction mechanism that allows riders to bid on a vehicle for a ride, but it does not allow multiple riders and cooperation between drivers.
%multiple riders and cooperation between drivers are not allowed \cite{Kleiner},
%\cite{Cheng2014} propose a mechanism for ridesharing that satisfies incentive compatibility, individual rationality and budget balance. However, they focus on the case where 
%all riders depart from the same origin and so their method does not coordinate the pickup schedules of riders at different locations \cite{Cheng2014}, 
%\cite{Zhao} propose a mechanism based on the Vickrey–Clarke–Groves (VCG) mechanism, but they do not explain how to compute the optimal vehicle allocations. Also, their mechanism satisfies budget balance only when there is no detour.
%budget balance is satisfied only when there is no detour \cite{Zhao},
%\cite{Crandall2001} propose an online posted-price mechanism 
%that is ex-post incentive compatible and budget balanced. However, their model only considers the case of autonomous vehicles (i.e. where vehicles can move without any drivers being allocated to that vehicle). Also, their allocation problem is NP-hard and cannot be solved in polynomial time.
%only the case of autonomous vehicles is considered \cite{Crandall2001},
%\cite{OstrovskyMichael2019} use cooperative game theory to analyze the optimal clustering of riders in ridesharing of autonomous vehicles. However, they only analyze the set of abstract trips and do not compute routes. 
%scalable computation of the optimal routes is not explained \cite{OstrovskyMichael2019},
%Other work using mechanism design focuses only on drivers \cite{Rheingans-yoo2019,LuAlicePeterI.Frazier2018,MaHongyaoFeiFang2019}.
%Different from our work, they do not consider the interesting and more flexible setting whereby a rider can be either a passenger or a driver.
%and some focus only on drivers %\cite{Rheingans-yoo2019,MaHongyaoFeiFang2019}.
\color{black}

%\cite{Cheng2014} focus on the case where all riders depart from the same origin, and so their method does not coordinate the pickup schedules of riders at different locations. Some studies mechanism design focusing only on the driver's side, which is different from our focus \cite{Rheingans-yoo2019,LuAlicePeterI.Frazier2018,MaHongyaoFeiFang2019}. Other studies propose approaches that are not scalable, and do not explain how to compute NP-hard allocation problem %\cite{Zhao,Crandall2001,OstrovskyMichael2019}.\cite{Crandall2001,OstrovskyMichael2019}}


%\cite{Kleiner} propose a second price auction mechanism that allows riders to bid on a ride and the drivers to choose the rider with the highest bid. The problem is that it does not allow multiple riders and cooperation between drivers. \cite{Cheng2014} propose a mechanism for ridesharing that satisfies incentive compatibility, individual rationality and budget balance. However, unlike our setting, they focus on the case where all riders depart from the same origin, and so their method does not coordinate the pickup schedules of riders at different locations. \cite{Zhao} propose a mechanism based on the Vickrey–Clarke–Groves (VCG) mechanism, but they do not explain how to compute the optimal vehicle allocations. Also, their mechanism satisfies budget balance only when there is no detour. \cite{Crandall2001} propose an online posted-price mechanism for autonomous vehicles that is ex-post incentive compatible and budget balanced. However, their allocation problem is NP-hard and cannot be solved in polynomial time. \cite{OstrovskyMichael2019} use cooperative game theory to analyze the optimal clustering of riders in ridesharing of autonomous vehicles. However, they only analyse the set of abstract trips and omit the routing computation.

%Some studies focus on mechanism design on the driver's side, which is different from our focus. Specifically, \cite{Rheingans-yoo2019} deal with a tractable macroscopic problem, \cite{LuAlicePeterI.Frazier2018} use a logit model to avoid combinatorial complexities, and  \cite{MaHongyaoFeiFang2019} formulate the problem as an ILP with an exponential number of variables.

In short, to date there exist no scalable mechanisms for general ridesharing settings that satisfy IC, IR and BB. To address this shortcoming, we make the following novel contributions:
\begin{itemize}
    \item We formulate a more general ridesharing problem compared to existing approaches. In particular, this is the first model that \modified{considers both autonomous and non-autonomous vehicles and where riders can switch between vehicles if it is beneficial to do so.} %In other words, it provides a way to design more dynamic and flexible public transportation than the current buses with fixed routes, which play an important role in suburban areas.}
    %allows agents to be both riders and drivers, considers manual as well as autonomous vehicles (where vehicles can drive to pick up riders without any agents being allocated to them), 
    %and where riders can switch vehicles.
    %, and where riders can switch vehicles if this is more efficient.
    %which, for the first time, takes into consideration fuel costs, as well as the driver's value of time, and includes both manual and autonomous vehicles as well as taxis for outside options. Unlike existing work, riders can also switch vehicles if this is more efficient.
    %\item We prove that, unsurprisingly, computing the optimal allocation is NP-hard. Nevertheless, by introducing some weak assumptions, we show that it can be to reduced to a polynomial-time linear program.
    \item \modified{We show that approaches based on VCG mechanisms or naive greedy (where riders are allocated in order of their marginal cost) do not satisfy the necessary properties. Specifically, the standard VCG approach does not satisfy BB and cannot be computed in polynomial-time. Also, naive greedy violates a property called monotonicity, meaning it fails to satisfy IC.}
    %Though the VCG mechanism can be computed efficiently with our algorithm, it fails to satisfy budget balance. Meanwhile, though it is possible to implement a budget balanced VCG mechanism, it sacrifices the efficient computation.
    %\item Using the algorithm, we propose a ridesharing mechanism based on the VCG mechanism that can be computed efficiently, but we show this is not (weakly) budget balanced. We therefore propose a budget balanced version of the VCG mechanism, but this comes at a higher computational cost.
    \item To address this, \modified{we propose a general methodology to design monotone greedy allocation mechanisms. We then apply this theory to produce a novel two-stage mechanism with carefully designed payments to ensure both IR and BB, as well as IC and scalability. }
    %we focus on greedy mechanisms. We clarify that mechanisms based on naive greedy allocations fail to satisfy truthfulness. Then
    %we characterize monotone allocations for greedy mechanisms, which is key in achieving truthfulness. 
    %We apply this approach to develop a greedy mechanism that is polynomial-time, truthful, individually rational and budget balanced.
    %According to \cite{myerson1983efficient}, no mechanism can achieve optimality, truthfulness, individual rationality and budget balance at the same time. In this sense, our mechanism achieves a theoretical limit and can be a standard mechanism for ridesharing.
	%\item To address this, we propose a budget balanced greedy-based mechanism that can be computed efficiently and show that it is monotonic and therefore incentive compatible.
%	\item We analyze the impact of autonomous vehicles replacing drivers on the usage of ridesharing systems.
	\item We empirically evaluate the performance of different mechanisms and show the advantages of our methods. Our monotone greedy mechanism satisfies all desirable properties with typically less than a 9\% social cost increase compared to the optimal allocation.
\end{itemize}
In what follows, Section~\ref{sec:model} introduces the ridesharing model and its mechanism design formulation. Section~\ref{sec:vcg} considers the VCG mechanism and its budget balanced version. Section~\ref{sec:greedy} studies the greedy mechanisms. Section~\ref{sec:exp} provides an empirical evaluation of the mechanisms and Section~\ref{sec:conclusions} concludes.  Due to space limitations, most proofs for the theoretical results are provided in \camera{the extended version of the paper}. 

%For the remainder of the paper, we start by presenting the ridesharing model, then present the VCG ridesharing mechanism followed by the budget balanced version. We then present a general theory to design monotone allocations for greedy mechanisms, and a greedy ridesharing mechanism. We conclude after presenting experimental results.

%For the remainder of the paper organized as follows. We start by presenting the ridesharing model. We then present the ridesharing mechanism based on the VCG mechanism and show the computational hardness result. Following this, we present the budget balanced version. \modaaai{We then present a general theory to design monotone allocations for greedy mechanisms, and apply the theory to design a greedy ridesharing mechanism.}
%We then present our experimental results. We conclude in the last section.
%Finally, the formulation of the ridesharing problem as a linear program is shown in the supplementary material.

\section{The Model}
\label{sec:model}
%Our objective is to design a mechanism that allocates vehicles to riders, calculates routes, and also computes payments to compensate for any detours and to incentivize truthful behaviour. 
In this section, we first provide a formal model of the ridesharing problem followed by an example. %\modaaai{The model is flexible enough to describe situations such that agents can be either riders or drivers, that vehicles need drivers or are autonomous, and that riders can switch vehicles on their way.} 
We then formulate this as a mechanism design problem.

\subsection{The Ridesharing (RS) Problem}
\label{sec:pmodel}

We assume finite time steps  $\mc{T}=\{0,1,\ldots,T\}$, set of riders  $\mc{N}=\{1,2,\ldots,N\}$ and vehicles $\mc{K}=\{1,2,\ldots,K\}$.  Let $w \in \mathbb{N}_{+}$ denote the vehicle capacity (i.e., the maximum number of riders in a vehicle). The road network is represented by a directed graph $\mc{G}=(\mc{V},\mc{E})$, where edges $\mc{E}$ denote road segments, vertices $\mc{V}$ denote locations, \modified{and loops $(v,v) \in \mc{E}$ are used to model stationary vehicles}.  
\modified{The length} of an edge $e\in \mc{E}$ is given by $l_{e}$ and denotes the travel distance. For simplicity \modified{we assume $l_{(v,v')}=1$ if $v\not=v'$, and $l_{(v,v)}=0, \forall (v,v')\in \mc{E}$.\footnote[1]{The former ensures that a rider is always at a vertex at each time step. Furthermore, since $l_{e}$ is used to compute costs (discussed below), the latter ensures that stationary vehicles do not incur fuel costs. Longer roads can be represented by joining multiple edges.}}
%We assume that the travel time of edge $e\in \mc{E}$ is equal to the length of the edge $l_{e} \in \mathbb{N}$.
Let $O_i^p,D_i^p \in \mc{V}$ denote the origin and the destination of rider $i\in \mc{N}$. Also, let $O_k^c$ denote the initial location of vehicle $k \in \mc{K}$, which does not have to be where riders are (in case of autonomous vehicles). We denote by $\mc{P}$  the set of all paths in $\mc{G}$. A \emph{path} is a vector of size $S$, denoted by $\langle v\rangle_S \equiv \langle v_1,\ldots,v_S\rangle$, where an element $v_s \in \mc{V}$ is the $s$-th location in the path and $(v_s,v_{s+1}) \in \mc{E}, \forall s < S$. Since paths do not include information of time, we define 
%, that have total travel time less than $T$.
a \emph{route} as a tuple of vectors $\langle \langle v\rangle_S,\langle t\rangle_S\rangle$ where the path departs from location $v_s$ at time $t_s$. Route $\langle \langle v\rangle_S,\langle t\rangle_S\rangle$ satisfies $t_{s+1} = t_{s}+l_{(v_s,v_{s+1})}$ if $v_s \not =v_{s+1}$. If $v_s=v_{s+1}$, it means the rider or vehicle stays at $v_s$ for an amount of time given by $t_{s+1}-t_s$ (e.g., to wait for a vehicle or because they already arrived at the destination). The set of routes is denoted by $\mc{R}$. The route of rider $i$ and the route of vehicle $k$ are denoted by $r_{i}^p, r_{k}^c \in \mc{R}$, respectively. 
We let ${\rm edge}(r,t) \in \mc{E}$ be a function that returns the edge in route $r$ that the rider or vehicle is traversing at $t$. E.g., ${\rm edge}(\langle \langle A,B,C\rangle,\langle 0,1,2\rangle \rangle,1)=(B,C)$.  Similarly, ${\rm loc}(r,t) \in \mc{V}$ returns the location at $t$. E.g., ${\rm loc}(\langle \langle A,B,C\rangle,\langle 0,1,2\rangle \rangle,1)=B$.
%We let ${\rm each}(r)$ be a function that returns a list of every $(e,t)$ included in route $r$, such that the rider or vehicle start traversing edge $e$ at $t$. 
Riders cannot move without vehicles but vehicles can move without riders if they are autonomous. If they are not autonomous, then they need at least one rider. %We do not always assume autonomous vehicles but only in some cases. 

We denote the \emph{assignment} of vehicles to riders with \modified{tensor} $B\in\mc{B}=\{0,1\}^{T\times N\times K}$. $B[t,i,k]=1$ is possible only if the path of rider $i$ is the same as vehicle $k$ at time $t$. %That is, a vehicle can be assigned to a rider for a move on edge, only when the departure timings are the same. 
The assignment may change over time, which means a rider can switch vehicles on the way\footnote[2]{In practice, this can take time, but we ignore this for simplicity. The model can  easily be extended by introducing waiting times for vehicles when riders switch \camera{at some designated safe areas}.}. We do not specifically distinguish between drivers and riders. Any rider in a vehicle can be a driver if the vehicle is not autonomous. Furthermore, riders can use a taxi as the outside option \modified{($B[t,i,k]=0,~\forall t\in\mc{T},k\in\mc{K}$)} if it is more beneficial than using ridesharing. We assume that the waiting time for a taxi is zero and the taxi takes the shortest path between the origin and destination of the rider. However, a rider cannot combine a taxi with ridesharing. 

An overall \emph{allocation} is denoted by
$\pi =\langle \vect{r}^p,\vect{r}^c,B \rangle \in \mc{R}^N\times\mc{R}^K\times\mc{B}$, where $\vect{r}^p=\langle r_{i}^p \rangle_{i\in\mc{N}}, \vect{r}^c=\langle r_{k}^c \rangle_{k \in \mc{K}}$ are the routes for riders and vehicles,  respectively. We will also use $r^p_i(\pi)$, $r^c_k(\pi)$ to denote a route for rider $i$ and vehicle $k$ given allocation $\pi$.  An allocation is feasible if, for each rider $i$, the route $r^p_i$ consist of a path between $O_i^p$ and $D_i^p$, and the vehicle capacity is not exceeded.  Formally, the set of \emph{feasible allocations} is defined by:

%\begin{equation*}
%\left.
\begin{align}
\Pi=&\{\langle \vect{r}^p,\vect{r}^c,B \rangle  \in \mc{R}^N\times\mc{R}^K\times\mc{B} |  \nonumber\\
&\forall t \in \mc{T}, i\in \mc{N}, k\in\mc{K}, r_i^p, r_k^c \in \mc{R}: \nonumber\\
 &{\rm loc}(r^p_i,0)=O_i^p,~{\rm loc}(r^p_i,T)=D_i^p,~{\rm loc}(r^c_k,0)=O_k^c, \nonumber\\
 & B[t,i,k]=1 \Rightarrow {\rm edge}(r_k^c,t)={\rm edge}(r_i^p,t),\nonumber\\
 & \exists t' \in \mc{T}, \forall k' \in \mc{K}: (B[t',i,k']=0, l_{{\rm edge}(r_i^p,t')}>0) \nonumber\\
 &\qquad \Rightarrow B[t,i,k]=0, \nonumber\\
&\sum_{i'\in \mc{N}}B[t,i,k]\leq w \}.
\end{align}
%\right.
%\label{eq:feas}
%\end{equation*}
The first line of constraints specifies origins and destinations of the routes. The second constraint is the definition of $B$. The third constraint means that a taxi cannot be combined with ridesharing (if riders traverse an edge using a taxi, they always use a taxi). The fourth is the capacity constraint.

If vehicles are not autonomous or have no dedicated driver, $\Pi$ needs an additional condition that any moving vehicle needs at least one rider: $l_{{\rm edge}(r_k^c,t)}>0 \Rightarrow \sum_{j\in \mc{N}}B[t,j,k]\modaaai{>} 0$.

Now that we have defined the allocation, we proceed with defining the costs which the system aims to minimise. These costs include travel and waiting time, fuel costs and taxi labour costs. Formally, the travel time of rider $i$ including waiting time is denoted by $T_i(\pi)=\min\{t_s|r_i^p=\langle \langle v\rangle_S,\langle t\rangle_S\rangle, v_s =D_i^p\}$\modified{, which is the earliest time to reach the destination}. Furthermore, let $T_i^0$ denote the travel time for rider $i$ using the shortest path (e.g., taxi).
%If ${\rm path}(O,D)$ denotes a shortest paths between $O \in \mc{V}$ and $D \in \mc{V}$, the shortest travel time of $i$ is denoted by $T_i^0=\sum_{e \in {\rm path}(O_i^p,D_i^p)}l_{e}$. 
The travel time of vehicle $k$ is denoted by 
$T_k^c(\pi)=\sum_{t \in \mc{T}}l_{{\rm edge}(r_k^c(\pi),t)}$.
%$T_k^c(\pi)=\sum_{(e,t) \in {\rm each}(r_k^c(\pi))}l_{e}$. 
Furthermore, let $\alpha,\beta \in \mathbb{R}$ denote the (additional) labour cost per time step for a taxi driver and fuel cost per distance for a vehicle, respectively. Let $\gamma_i \in \Gamma=[0,\gamma_{max}]$ represent the value of time, i.e., a subjective  cost rider $i$ is willing to pay to avoid a unit of travel time. Then the cost of rider $i$ is: $c_i(\pi)=c_i^0=(\alpha+\beta+\gamma_i)T_i^0$ when using a taxi, and $c_i(\pi)=\gamma_{i}T_i(\pi)$ when using ridesharing.   In addition, the fuel cost of the ridesharing system is calculated separately and is given by $c_F(\pi)=\sum_{k \in \mc{K}}\beta T_k^c(\pi)$. Given this, the {\it ridesharing (RS) problem} is to find a feasible allocation $\pi\in\Pi$ that minimizes the social cost including fuel cost $C_F(\mc{N},\pi)=\sum_{i \in \mc{N}}c_i(\pi)+c_F(\pi)$.


%\subsection{Example}
%\commenteg{The figure does not really contain much information. For example, it does not show $T=3$ or anything to do with time or the allocation. Can we include additional information such as the allocation/assignment, or more notation to make the figure more useful? Otherwise we might get similar comment to before. Finally, the graph seems a directional graph, but don't see this mentioned before in the model.}
To illustrate the model, \modified{Figure \ref{fig:tradgreedy} shows an example with $N=2, K=2$ and $T=5$. The two figures show two possible allocations: in left figure, for example, $r_1^p=\langle \langle A,A,B\rangle,\langle 0,3,4\rangle \rangle$  and $ r_2^p=\langle \langle B,B,C\rangle,\langle 0,1,2\rangle \rangle$. Rider 2 is assigned to vehicle 1 at $t=1$, i.e., $B[1,2,1]=1$ while rider 1 is not assigned to vehicle 2  until $t=3$, i.e., $B[3,1,2]=1$. If $\gamma_1=2$ and $\gamma_2=1$, then the optimal allocation is the one on the right, with $T_i=T_k^c=3$ and social cost $C_F=15$.}

\subsection{Mechanism Design Formulation}
\label{sec:mmodel}
%
A mechanism takes reports from riders on their privately-known types as input, and computes the allocation and payment as output. In our model, we assume $O_i^p$ and $D_i^p$ are easy to track \modified{with GPS} and so $\gamma_i$ is the only private information, which is referred to as rider $i$'s \emph{type}. Let $\vect{\gamma}\in \Gamma^N$ be the type profile of all riders, $-i$ the set of riders except for $i$, and $\vect{\gamma}_{-i}$ the types of all riders except $i$.
%(in theory, riders could misreport the destination and walk to $D_i^p$, but such a manipulation would normally be very costly)
%$\theta_i=(O_i^p,D_i^p,ta_i,\gamma_i)$. $ta_i \in \mc{T}$ is the latest acceptable arrival time.
For simplicity, we assume that all riders and vehicles are ready to depart at $t=0$, but this can be easily extended.  %
%$\Theta$ denotes the set of types and 
%
A \emph{mechanism} is then defined as a function $\mc{M}:\Gamma^N \to \Pi \times \mathbb{R}^N$, that  computes a feasible allocation $\pi \in \Pi$ from a given type profile and payment vector $\vect{x}(\pi)\in \mathbb{R}^N$, where $x_i(\pi)$ is the payment of rider $i$ to the system. We sometimes use  $\pi(\vect{\gamma})$ to emphasize the dependence on  $\vect{\gamma}$. If $i$ chooses a taxi, $x_i(\pi)=0$.  Sometimes we use short-hand notation $\pi(\gamma_i)=\pi(\gamma_i,\vect{\gamma}_{-i})$.
%and $\pi_{-i}=\pi(\vect{\gamma}_{-i})$. 
Given this, the utility of rider $i$ is defined as $u_i(\pi)=-c_i(\pi)-x_i(\pi)$. 
%Since type $\vect{\gamma}$ is private information, the mechanism receives reports $\hat{\vect{\gamma}}\in \mathbb{R}_{+}^N$ from riders as inputs. 

\camera{In practice, the ridesharing mechanism may work as in the following example. First, rider $i$ reports their type $\gamma_i$ using a slider in a suitable smartphone app, along with $O_i^p$ and $D_i^p$. Note that $\gamma_i$ is not necessarily truthful. Once the report profile $\vect{\gamma}$ is obtained, the mechanism computes $\pi(\gamma)$ and $\vect{x}(\pi)$, and reveals them to riders before travel. 
%If rider $i$ accepts the offer, the service is executed and $x_i$ is charged.
Finally, $x_i$ is charged after the travel.}
\camera{To this end}, the mechanism \camera{needs} to achieve the following properties:

%\begin{itemize}
    %\item 
    Budget balance (BB), which is formulated as:
    \begin{equation}
\sum_{i \in \mc{N}}x_i(\pi)\ge c_F(\pi).
\end{equation}

    %\item 
    Individual rationality (IR), which is formulated as:
%
\begin{equation}
u_i(\pi)\ge-c_i^0, ~\forall i \in  \mc{N}.
\label{eq:ir}
\end{equation}

Dominant-strategy incentive compatibility (DSIC), or truthfulness, which is formulated as:
\begin{equation}
 \left.
 \begin{array}{l}
u_i(\pi(\gamma_i,\vect{\gamma}_{-i}))\ge u_i(\pi(\gamma_i',\vect{\gamma}_{-i})), \\
~\forall \gamma_i' \in \Gamma,  ~\forall i \in  \mc{N}, \forall \gamma_{-i} \in \Gamma^{N-1}.
 \end{array}
 \right.
\end{equation}
 
%\modified{Note that we look at a fleet of vehicles owned by a company, and focus on the total revenue of the company , rather than the individual budget valance for each vehicle.}
 
\section{The VCG Mechanisms}
\label{sec:vcg}

%We start by considering 
\modified{Next, we will show that the well-known VCG mechanism \cite{Shoham2008} does not achieve BB and polynomial-time computation at the same time when applied to the RS problem.} This mechanism first computes an optimal allocation $\pi(\vect{\gamma})$ given (reported) type profile $\vect{\gamma}$ and then it computes the payment $\vect{x}(\pi)$ as the externality that each rider imposes on other riders. Specifically, for our RS problem, the objective is to minimize $C_F(\mc{N},\pi)$, and so the VCG payment is computed as $x_i(\pi)=C_F(-i,\pi(\vect{\gamma}))-C_F(-i,\pi(\vect{\gamma}_{-i}))$. As a result, the optimal allocation $\pi$ and the payment $\vect{x}$ guarantee DSIC and IR. %The optimal allocation $\pi(\vect{\gamma})$ and $\pi(\vect{\gamma}_{-i})$ can be computed by solving the RS problem. 
%\modified{In the supplementary material, we show that the RS problem is NP hard, but with a mild assumption, an algorithm based on integer linear program (ILP) can solve it in polynomial time. However, VCG has the following issue.}
However, we show that the RS problem is NP hard by reducing the travelling salesman problem. Also, VCG has the following issue.
\begin{comment}
\camera{In the extended version, we show that the RS problem is NP hard by reducing the travelling salesman problem. However, with a mild assumption, an algorithm based on integer linear program (ILP) can solve it in polynomial time. The algorithm relaxes the ILP into a linear program (LP), that outputs an integer solution of the original ILP. The detail of the algorithm and proofs are also in the extended version. However, VCG has the following issue.}
\end{comment}

\begin{minortheorem}
\modified{VCG does not satisfy BB in the RS problem.}
\end{minortheorem}
%\commenteg{I SEEM TO RECALL THAT REVIEWERS DIDN'T LIKE THIS FIGURE SINCE IT WAS NOT VERY INFORMATIVE. COULD REMOVE IT IF NEEDED}
%\modified{The proof is done with the following counterexample.}
\begin{proof}
Suppose both riders 1 and 2 have the same origin $O$ and destination $D$, which are directly connected with an edge. VCG allocates the vehicle to both riders for sharing. Since the absence of either rider does not change the allocation and cost of the other rider, the VCG payment is zero for both riders. This means the fuel cost of the vehicle is not recovered.
\end{proof}

\modified{Despite this negative result, we show it is possible to modify VCG to satisfy BB by sacrificing the optimality, as follows.} Let $\mc{K}_i(\pi)=\{k \in \mc{K} |B[t,i,k]=1, \exists t \in \mc{T}\}$ denote the set of vehicles that rider $i$ uses. Then, the total fuel costs of all rides that a rider $i$ is involved in is $c_F^i(\pi)=\sum_{k \in \mc{K}_i}\beta T_k^c(\pi)$. We then define an \emph{imaginary} system cost by redundantly counting the fuel costs of vehicles as follows: $c_I(\pi)=\sum_{i \in \mc{N}}c_F^i(\pi)$. The total social cost including this imaginary cost is then given by $C_I(\mc{N},\pi)=\sum_{i \in \mc{N}}c_i(\pi)+c_F(\pi)+c_I(\pi)$. 
Given this, we have a budget balanced VCG (BVCG) %First, the mechanism computes an allocation $\pi$ 
by replacing the objective function of VCG with $C_I$. 
\begin{minortheorem}
\modified{Assuming autonomous vehicles, BVCG satisfies DSIC, IR and BB.}
\end{minortheorem}
\modified{Briefly, this is because the payment is computed based on the imaginary cost $c_I$, which is redundant and larger than $c_F$. Autonomous vehicles guarantee the feasibility of vehicle routing even when $i$ is absent in the payment computation. However, scalability is an issue as the standard VCG.}
%Since the new objective function with $C_I$ is a non-linear function, we cannot use the ILP based polynomial-time algorithm.}

\section{Greedy Mechanisms}
\label{sec:greedy}

\modified{To address the issues with VCG mechanisms,} we consider greedy mechanisms in this section.  
%\modified{However, as we will see, mechanisms based on naive greedy allocations fail to satisfy DSIC.}
%we cannot be formulated as a linear function as $C_F$ and 
%then we cannot use the same efficient algorithm in . Hence, for large settings, we require another mechanism that can compute a budget balanced allocation efficiently.
To this end, we first show that a naive greedy approach does not satisfy IC and we 
%brief the existing theory of mechanism with one parameter agents. Then we 
propose a general theory to design greedy DSIC mechanisms based on the concept of monotonicity. Then, we apply our theory to design a greedy DSIC ridesharing mechanism.

\subsection{Monotonicty and Violation with Naive Greedy}
\label{sec:naivegreedy}

\cite{Myerson1981,archer2001truthful} showed that, for single-valued domains, monotonicity of the allocation function $\pi(\vect{\gamma})$ is a necessary and sufficient condition for the existence of  payments $\vect{x}(\pi)$ satisfying DSIC. Using notation from our model, monotonicity is defined as follows:
%
\begin{equation}
    \gamma_i \leq \gamma_i' \Rightarrow V_i[\pi(\gamma_i)] \leq V_i[\pi(\gamma_i')], ~\forall \gamma_i, \gamma_i' \in \Gamma,
    \label{eq:mono}
\end{equation}
where, in general, $V_i:\Pi\to \mathbb{R}$ is the amount allocated, and referred to as \emph{work} in \cite{archer2001truthful} and, for our setting, $V_i=-T_i(\pi)$ corresponds to the negative travel time. 

Although monotonicity plays a key role in designing DSIC mechanism, finding appropriate monotone allocation functions $\pi$ is non-trivial. \modified{Here, we show that a naive approach fails to implement a DSIC mechanism. We define a naive greedy allocation as follows. First, all riders are assigned to a taxi by default. Then, for each iteration it chooses rider $i$ who 
%reduces the social cost by the most, i.e., the one that minimizes
minimizes the marginal social cost, given by 
$c_i-c_i^0+c_F$, without changing the allocation in riders allocated so far, and computes the best allocation for the current rider.}


\begin{figure}[t]
\centering
\includegraphics[width=1.\columnwidth]{fig/tradgreedy2.pdf}
\caption{\modified{Example showing how monotonicity is achieved with our mechanism and violated with a naive greedy mechanism: $D_1^p=B,D_2^p=C,O_1^c=C,O_2^c=D$. Assume $l_e=1, \forall e\in \mc{E}$ and expensive taxi $\alpha=10$ and $\beta=1$.}}
\label{fig:tradgreedy}
\end{figure}


\begin{minortheorem}
\modified{Mechanisms based on the naive greedy allocation do not satisfy monotonicity or DSIC.}
\label{thm:naivegreedy}
\end{minortheorem}

\begin{proof}
\modified{Figure \ref{fig:tradgreedy} also shows a counterexample whereby a naive greedy allocation fails to satisfy monotonicity. Let $\gamma_2=4$. If $\gamma_1=3$, the naive greedy allocates vehicle 1 to rider $2$ in the first iteration because the rider brings the lowest cost $\gamma_2 T_2-(\alpha+\beta+\gamma_2)T_2^0+c_F=-5$ (left figure). However, if $\gamma_1=1$, the cost of the rider decreases as $\gamma_1 T_1-(\alpha+\beta+\gamma_1)T_1^0+c_F=-6$ and rider $1$ is allocated first (right figure). Then, the lower $\gamma_1$ results in the earlier allocation and larger $V_1=-T_1$, which is the violation of the monotonicity (\ref{eq:mono}). This violation of monotonicity means mechanisms with the naive greedy allocation also violate DSIC, since this is a necessary condition for DSIC.}
\end{proof}


\subsection{Design of Monotone Greedy Allocation}
\label{sec:theory}

To \modified{address the issue above}, we propose a characterisation that is useful for designing monotone allocation functions for greedy mechanisms. \modified{As we saw, the naive greedy violates monotonicity by giving priority to the riders with lower $\gamma_i$.}
%In more detail, a greedy mechanism is a mechanism which allocates agents one at a time. 
\modified{Instead, we allocate agents}
%Importantly, the agents are allocated 
in descending order of their (reported) type $\gamma_i$.
%order of the agents is determined by their (reported) type $\gamma_i$ \modaaai{in descending order.}, and an agent with a higher $\gamma_i$ is allocated earlier. 
In what follows, we use the index to denote the order in which agents are allocated.  I.e., $j<i$ implies $\gamma_j \geq \gamma_i$ and that $j$ is allocated before $i$. Let $\pi_{\leq i}$ denote the allocation up to and including $i$ (with remaining agents allocated arbitrarily or, e.g., in the context of ride sharing, allocated to a taxi). 
%$<i=\{j\in\mc{N}|\gamma_j>\gamma_i\}$ denote the set of agents prior to $i$, and $j<i$ denotes that $j$ is an element of $<i$.
%Also, let $\Pi_{\mc{M}}\subseteq \Pi$ be the feasible set where $\mc{N}\setminus\mc{M}$ are unallocated (or allocated to an outside option). Then, a partial allocation for prior agents is denoted by $\pi_{<i} \in \Pi_{<i}$. 
Also, let $\Pi_{\leq i}(\pi_{\leq i-1})$ or simply $\Pi_{\leq i}$ denote the set of possible allocations given $\pi_{\leq i-1}$, keeping agents $j<i$ fixed. 
%\begin{equation}
%\left.
%\begin{array}{ll}
%\Pi_{\leq i}(\pi)&=\{\pi_{\leq i} \in %\Pi_{\leq i} |  \\
%& \pi_{\leq i} {\rm ~is ~same ~as~ } \pi, %\forall j<i \}.
%\end{array}
%\right.
%\label{eq:greedyfeas}
%\end{equation}
%Then, the set of allocations for $i$ based on a prior allocation $\pi_{<i}$ is defined as $\Pi^i=\Pi_{\leq i}(\pi_{<i})$. 
%With slight abuse of notation, we sometimes use $\Pi_{\leq i}(\gamma_i)$ to emphasize the dependence on $\gamma_i$. We require shrinking allocation space, $\Pi^i\subseteq \Pi^j$ if $j<i$.
%We will see a specific definition for the ridesharing problem in the next section.
%Also, let $\Pi_i$ be the set of feasible allocations of agent $i$, given all the allocations made so far, and $\pi_i\in \Pi_i$ is an allocation. We will use $\pi_i(\gamma_i)$ and $\Pi_i(\gamma_i)$ to emphasize the dependence on $\gamma_i$. $\Pi_{j\leq i}$ is the set of allocations of the riders up to $i$ and $\pi_{\leq i}\in \Pi_{j\leq i}$ is an allocation.
Given this, we define a class of \emph{greedy allocations with decreasing choices (GADC)} as follows:
%Let us denote a subset of agents $\mc{N}'\subseteq \mc{N}$ and let $\Pi_i$ and $\Pi_{\mc{N}'}$ be the set of feasible allocations of agent $i$ and set of feasible allocations of agents $\mc{N}'\subseteq \mc{N}$, respectively. For simplicity, we denote a set of agents $(j\leq i)=\{j\in\mc{N}|\gamma_j\leq\gamma_i\}$, and an allocation of those agents $\pi_{\leq i} \in \Pi_{j\leq i}$. Given this, we define a class of greedy allocations with decreasing choice (GADC) as follows:
%
\begin{equation}
\left.
\begin{array}{l}
    %\pi_{\leq i}=\underset{\substack{\pi \in\Pi^i}}{\argmin}J(\pi)
    \pi_{\leq i}=\argmin_{\pi \in \Pi_{\leq i}} J(\pi)
\end{array}
\right.
\label{eq:gars}
\end{equation}
subject to $\Pi_{\leq i} \subseteq \Pi_{\leq {j}}$ if $j<i$. Here,  $J:\Pi\to \mathbb{R}$ is an objective function. In words, GADC captures allocation functions which compute the optimal allocation for each $i$ individually given a set of possible allocations, \emph{and this set reduces as $i$ reports a smaller $\gamma_i$} (and so appears later in the sequence).
%The constraint means that the set of options reduce when an agent reports a smaller value and so is allocated later. Then:% the following theorem holds.

\begin{theorem}
    Let $\pi_{\leq i}(\gamma_a),\pi_{\leq i}(\gamma_b)$ denote $i$'s allocation when reporting $\gamma_a$,$\gamma_b$ respectively. A GADC satisfies monotonicity if and only if, $\forall \gamma_a, \gamma_b, i \in \mc{N}$:
    \begin{equation}
%\left.
%\begin{array}{l}
    J(\pi_{\leq i}(\gamma_a))\leq J(\pi_{\leq i}(\gamma_b)) 
    \Rightarrow V_i[\pi_{\leq i}(\gamma_a)]\geq V_i[\pi_{\leq i}(\gamma_b)]. 
%\end{array}
%\right.
    \label{eq:consist}
    \end{equation}
    \label{thm:nsmono}
\vspace{-0.2cm}
\end{theorem}
Intuitively, this means that, the more an agent contributes to decreasing the global objective (in our case, minimising the social cost), the better their allocation should be (in our case, the lower the travel time).  
%\modified{Briefly, this is because the condition (\ref{eq:consist}) means the minimization of $J$ by GADC coincides with the maximization of $V$, and riders with larger $\gamma$ has higer priority to be allocated more.}


\subsection{Monotonic Greedy Ridesharing Mechanism}
\label{sec:greedyrs}

We now apply Theorem~\ref{thm:nsmono} to our setting. First, we customize GADC from section \ref{sec:theory} for our ridesharing problem. In particular, $\Pi_{\leq i}(\pi)$ 
%in (\ref{eq:greedyfeas}) 
is redefined as follows:

\begin{align}
\Pi_{\leq i}(\langle \vect{r}^p,\vect{r}^c,B \rangle) & =\{ \langle \vect{r'}^p,\vect{r'}^c,B' \rangle \in \Pi | \nonumber\\
&\forall t \in \mc{T}, j<i,j'>i, k \in \mc{K}: \nonumber\\
& B'[t,j,k]=B[t,j,k], {r'}^p_j=r^p_j, 
\label{eq:shrink}\\
& B[t,j',k]=0 \}.
\label{eq:greedyfeasrs}
\end{align}

This means that, when computing $i$'s allocation, the allocation of the prior riders $j<i$ are not changed. With this definition, the assumption $\Pi_{\leq i}\subseteq \Pi_{\leq j}$ holds, because \modified{constraint (\ref{eq:shrink})} 
%the first constraint for $\forall j<i$ 
shrinks the set.
%, while the second constraint does not, due to the unlimited supply of taxi.
Then, a greedy allocation for ridesharing is obtained by applying equation (\ref{eq:gars}), with the objective function $J(\pi)=\sum_{i\in \mc{N}}c_{i}(\pi)$. \modified{In addition, to obtain monotonicity,  (\ref{eq:consist}) must be satisfied. To this end, we will show that we require an additional constraint whereby riders cannot be allocated to a taxi (i.e., their outside option). Although this constraint seems restrictive, we will relax this again later so that riders can use taxis if this is in their best interest (to satisfy IR). In the following, we refer to this setting as greedy allocation for ridesharing with no-taxi constraint or \mbox{GARS-N}. Formally:}
\begin{equation}
\left.
\begin{array}{l}
\pi_{\leq i}=\underset{\substack{\pi \in\Pi^i}}{\argmin}\underset{\substack{i'\in \mc{N}}}{\sum}c_{i'}(\pi) \\
s.t.~l_{{\rm edge}(r_i^p,t)}>0\Rightarrow \underset{\substack{k \in\mc{K}}}{\sum} 
B[t,i,k]=1, \forall t\in \mc{T}. \\
\end{array}
\right.
\label{eq:gars_notaxi}
\end{equation}


\begin{lemma}
GARS-N satisfies monotonicity.
\label{thm:gars_nmono}
\end{lemma}

\modified{Briefly, this is because minimizing $J$ coincides with minimizing $c_i$ for each rider $i$, since the constraints (\ref{eq:shrink}) and (\ref{eq:greedyfeasrs}) do not allow $i$ to change the allocations and costs of other riders. If riders do not use a taxi, $V_i=-T_i$ is proportional to $c_i$ and the equivalent condition of monotonicity in Theorem \ref{thm:gars_nmono} is satisfied. With the case in Figure \ref{fig:tradgreedy}, GARS-N allocates rider 1 first (right figure) when $\gamma_1=5$ and $\gamma_2=4$, and then $T_1=3$. Meanwhile, if $\gamma_1=1$, rider 2 is allocated first (left figure) and then $T_1=4$. Contrary to the naive greedy, the higher $\gamma_1$ results in the earlier allocation and larger $V_1$, and this satisfies monotonicity. Note that, without the no-taxi constraint, monotonicity can be violated as follows. If a taxi is cheap ($\alpha=1$), then rider 1 uses a taxi when $\gamma_1=1$, resulting in $T_1=1$, which violates monotonicity. Also, note that the no-taxi constraint does not help  naive greedy because nobody uses a taxi in the proof of Proposition \ref{thm:naivegreedy}.}


Next, we consider the computation of the payment.  Let $\hat{T}_i(\pi)=T_i(\pi)-T_i^0$ denote the normalized travel time. Following \cite{Myerson1981}, the unique payment satisfying DSIC is given by:
\begin{equation}
    x_i = x_i^0+\int_0^{\gamma_i} \gamma \frac{d}{d\gamma}\hat{T}_i(\pi(\gamma)) d\gamma
	\label{eq:integ}
\end{equation}
%
 where $x_i^0$ is a value which is independent of $i$'s report.  Solving the integral is challenging in general since it is necessary to recompute the allocations given all possible types of the rider whose payment we are computing. However, in our case, because $\hat{T}_i(\pi)$ only depends on the order of the allocation, it is sufficient to vary the position in the ordering. We refer to the GARS-N allocation with this payment as the GARS-N mechanism. Also, this mechanism can be computed in polynomial-time because the problem (\ref{eq:gars_notaxi}) includes the computation of a single rider only with the routes of former riders fixed, and is not NP-hard.
 %using the same technique \modified{in section \ref{sec:vcg}}.  

\begin{lemma}
The GARS-N mechanism is DSIC and can be computed in polynomial-time.
\label{thm:garsn_dsic}
\end{lemma}

To ensure BB, we compute the base payment $x_i^0$ based on report independent parameters $\vect{T}_0$, $\hat{\vect{T}}_{min}$ and $c_{Fub}$, where $\vect{T}_0$ is a vector of $T_i^0$. Furthermore,  $\hat{\vect{T}}_{min}$ is a vector of normalized minimal travel times, which is computed by solving the following allocation problem:
%
\begin{equation}
\left.
\begin{array}{l}
\pi=\underset{\substack{\pi' \in\Pi}}{\argmin}\underset{\substack{i\in\mc{N}}}{\sum}\hat{T}_i(\pi') \\
s.t.~l_{{\rm edge}(r_i^p,t)}>0\Rightarrow \underset{\substack{k \in\mc{K}}}{\sum} 
B[t,i,k]=1, \forall t\in \mc{T}, \forall i \in \mc{N}.\\
\end{array}
\right.
\nonumber
%\label{eq:minT}
\end{equation}
%
Finally, $c_{Fub}$ is an upper bound on the fuel cost $c_F$ of \mbox{GARS-N}. We assume that this parameter is given (in the experimental section, we explain how this is computed in our experimental setting).
%computed by solving GARS-N with all allocation orders that the orders of two riders are changed from the report. Due to the limited space, complete algorithm is explained in the full paper.
The base payment is computed by splitting $c_{Fub}$ among riders,
proportional to \modaaai{each agent $i$'s relative shortest travel time, $T^0_i - \hat{T}_{min,i} - \min_j (T^0_j - \hat{T}_{min,j})$.} %$\vect{T}^0-\hat{\vect{T}}_{min}-\min(\vect{T}^0-\hat{\vect{T}}_{min})$.
%. Riders with longer trips and less waiting time pay more. For this purpose, it computes the normalized minimum travel time (line \ref{alg:bp.t},\ref{alg:bp.nt}) and makes the base payment proportional to it (line \ref{alg:bp.coef},\ref{alg:bp.prop}). 
Since this base payment covers $c_{Fub}$, GARS-N is BB.

\color{black}

\begin{lemma}
If $c_{Fub}$ is given, the GARS-N mechanism is budget balanced.
    \label{thm:gbb}
\end{lemma}


\begin{comment}
\removable{
\begin{proof}[Proof of Lemma \ref{thm:gbb}]
From the base payment computation \textproc{BasePayment}, and since $\Delta \vect{x}\geq \vect{0}$,
\begin{equation}
\underset{\substack{i \in \mc{N}}}{\sum}x_i \geq \underset{\substack{i \in \mc{N}}}{\sum}x_i^0 = c_{Fub} \geq c_{F}.
\label{eq:gbbp}
\end{equation}
\end{proof}
}

\begin{algorithm}                    
	\caption{Base Payment}
	\label{alg:bp}
	\begin{algorithmic}[1]
		\Output Base payment $\vect{x}_0$
		\Procedure{$\vect{x}_0=$BasePayment}{$\hat{\vect{T}}_{min},c_{Fub}$}
		\State{Compute loss: $\Delta \vect{T}=\vect{T}^0-\hat{\vect{T}}_{min}$} \label{alg:bp.t}
		\State{Normalization: $\Delta \vect{T}=\Delta \vect{T}-\min(\Delta \vect{T})$} \label{alg:bp.nt}
		\If{$\sum(\Delta \vect{T})==0$}
		    \State{$x_i^0=c_{Fub}/N, ~\forall i \in \mc{N}$}
		\Else
		    \State{$k=c_{Fub}/\sum(\Delta \vect{T})$} \label{alg:bp.coef}
		    \State{$x_i^0=k\Delta T_i,~\forall i \in \mc{N}$} \label{alg:bp.prop}
		\EndIf
		\EndProcedure
	\end{algorithmic}
\end{algorithm}
\end{comment}

%\modaaai{The proof is in Appendix B.}
We now discuss IR. Since the no-taxi constraint restricts outside options, it can cause the violation of IR in some settings. To address this issue, we use the following lemma.
%(the proof is \modaaai{in  Appendix B}).
%(The proof is omitted and shown in the full paper.)

\begin{lemma}
The GARS-N mechanism satisfies IR if
\begin{equation}
    \hat{T}_i(\pi(0))\leq [(\alpha+\beta)T_i^0-x_i^0]/\gamma_{max}, ~\forall i \in \mc{N}.
\label{eq:irs}
\end{equation}
\label{thm:irs}
%\vspace{-0.2cm}
\end{lemma}

\begin{comment}
\begin{proof}[Proof of Lemma \ref{thm:irs}]
\begin{equation}
\left.
\begin{array}{l}
[(\alpha+\beta)T_i^0-x_i^0]/\gamma_{max}\geq \hat{T}_i(\pi(0))\\
\therefore (\alpha+\beta)T_i^0\geq \gamma_{max}\hat{T}_i(\pi(0))+x_i^0\geq \gamma_i\hat{T}_i(\pi(0))+x_i^0\\
\therefore (\alpha+\beta)T_i^0-\gamma_i\hat{T}_i(\pi)\geq  \gamma_i[\hat{T}_i(\pi(0))-\hat{T}_i(\pi)]+x_i^0 \geq x_i(\pi)\\
\therefore (\alpha+\beta+\gamma_i)T_i^0\geq \gamma_iT_i(\pi)+x_i(\pi)\\
\therefore c_i^0\geq c_i(\pi)+x_i(\pi)\\
\end{array}
\right.
\end{equation}
\end{proof}
\end{comment}

%\vspace{-0.2cm}
%The proof is in Appendix B. 
Briefly, (\ref{eq:irs}) shows the lower bound of the cost that satisfies IR.
We can now define the GARS-N mechanism with individual rationality (GARS-NIR) as follows. Before executing GARS-N, riders that violate condition (\ref{eq:irs}) are excluded from the mechanism, and are allocated to a taxi. This process is repeated until there is no violation. Then GARS-N is executed with the remaining riders. Since no riders violate (\ref{eq:irs}), this mechanism satisfies IR. 

\color{\cameracolor}
Algorithm \ref{alg:gnir} shows the pseudocode of GARS-NIR (using Python-like list operations). It filters out riders who violate IR condition (\ref{eq:irs}) in line \ref{alg:gnir.filter} and allocates them to a taxi (line \ref{alg:gnir.taxi}). Then, \textproc{GARS-N} in Algorithm \ref{alg:gn} computes the allocation for riders who satisfy (\ref{eq:irs}). First, it sorts riders in descending order of reported $\gamma_i$ (line \ref{alg:gn.sort}). Then it computes an allocation by \textproc{GreedyAlloc} (line \ref{alg:gn.alloc}). From line \ref{alg:gn.pay1} to \ref{alg:gn.pay0}, it computes the second term of $x_i$ in (\ref{eq:integ}), by changing the order of riders. In line \ref{alg:gn.pay1}, variables are initialized. For each rider $i$ (line \ref{alg:gn.for1}), it changes the order of the rider (line \ref{alg:gn.for2} to \ref{alg:gn.ord2}) and the report with a consistent value $\gamma_i'$ (line \ref{alg:gn.gamma}), and computes an allocation with the new order $\mc{N}'$ (line \ref{alg:gn.newalloc}). Thus, the integral term in (\ref{eq:integ}) is computed (line \ref{alg:gn.integ}), and the payment $x_i$ is given by adding the base payment $x_i^0$ (line \ref{alg:gn.pay0}).
The \textproc{GreedyAlloc} function (Algorithm \ref{alg:ga}) computes the allocation for each rider one by one by solving (\ref{eq:gars_notaxi}) in line \ref{alg:ga.solve}. 


%, for each rider $i$, the mechanism changes the priority of $i$ (line \ref{alg:gm.ord1}-\ref{alg:gm.ord2}), and computes the allocation with the new order in line \ref{alg:gm.newalloc}. The payment of rider $i$ is computed by adding the change in allocation $\hat{T}_i$ (line \ref{alg:gm.pay}). What is done here is the integral computation of monotone function $\hat{T}_i(\gamma_i)$ as (\ref{eq:integ}). Since $\hat{T}_i(\gamma_i)$ only depends on the allocation order, it changes only when the order changes and then shapes like a staircase as in Fig \ref{fig:gic}.

%For each iteration, a rider $i^*$ is selected (line \ref{alg:ga.iter}), and added into a set riders $\mc{N}_g$ (line \ref{alg:ga.add}). The algorithm solves a ridesharing problem $RS^*$ in each iteration to update the allocation (line \ref{alg:ga.solve}). $RS^*$ has the set of riders $\mc{N}_g$, the set of vehicles $\mc{K}$. %EG COMMENT: Don't understand this last sentence
%Besides, two constraints are applied. One is the constraint of no taxi as mentioned before. This is formalized as $(t,e)\in r_k^c, ~\forall (t,e=(o,d\not=o)) \in r_i^p,~\forall i \in \mc{N}_g, \exists k \in \mc{K}$, which in words, a vehicle is allocated to every move of the riders. The other is a constraint to fix the allocation of riders in the last iteration $\vect{\pi}_{last}$. This is formalized as $r_j^p=r_j^p(\vect{\pi}_{last}), ~\forall j<i^* \in \mc{N}_g$.


\begin{algorithm}[t]                 
	\caption{GARS-NIR}
	\label{alg:gnir}
	\begin{algorithmic}[1]
		%\Input Ordered set of riders $\mc{N}$
		%\Output Allocation $\vect{\pi}$
		\Procedure{$\pi=$GARS-NIR}{$\vect{\gamma},\mc{N}$}
		\State{$\mc{N}_{IR}=[]$}
		\For{$i \in \mc{N}$} \label{alg:gnir.iter}
		\If{$i$ satisfies (\ref{eq:irs})}
		\label{alg:gnir.filter}
		\State{$\mc{N}_{IR}.{\rm append}(i)$} 
		\Else
		\State{$B[t,i,k]=0,~\forall t \in \mc{T},\forall k\in\mc{K}$}
		\label{alg:gnir.taxi}
		\EndIf
		\EndFor
		\State{Return \textproc{GARS-N($\vect{\gamma},\mc{N}_{IR}$)}}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]                 
	\caption{GARS-N}
	\label{alg:gn}
	\begin{algorithmic}[1]
		%\Input Report $\vect{\gamma}$
		%\Output Allocation $\pi$, Payment $\vect{x}$
		\Procedure{$(\pi,\vect{x})=$GARS-N}{$\vect{\gamma},\mc{N}$}
		\State{$\hat{\mc{N}}=$Sorted $\mc{N}$ in descending order of $\gamma_i$} \label{alg:gn.sort}
		\State{$\pi=\textproc{GreedyAlloc}(\vect{\gamma},\hat{\mc{N}})$} \label{alg:gn.alloc}
		\State{$t_i=\hat{T}_i(\pi),\Delta x_i=0,  \forall i \in \mc{N}$} \label{alg:gn.pay1}
		%\State{Initialize upper bound of fuel cost: $c_{Fmax}=c_F(\pi)$}
		\For{$i \in \mc{N}$} \label{alg:gn.for1}
		\For{$order_i \in [\hat{\mc{N}}.index(i),\ldots,N]$}
			\label{alg:gn.for2}
    		\State{$\mc{N}'=\hat{\mc{N}},\vect{\gamma}'=\vect{\gamma}$}
        	\State{$j=\hat{\mc{N}}[order_i]$}
			\State{$\mc{N}'.{\rm pop}(\hat{\mc{N}}.index(i))$}
			\State{$\mc{N}'.{\rm insert}(order_i,i)$}
			\label{alg:gn.ord2}
			\State{$\gamma_i'=\gamma_j$}
			\label{alg:gn.gamma}
    		\State{$\pi'=\textproc{GreedyAlloc}(\vect{\gamma}',\mc{N}')$} \label{alg:gn.newalloc}
    		\State{$\Delta x_i=\Delta x_i+(\hat{T}_i(\pi')-t_i)\gamma_j$} \label{alg:gn.integ}
    		\State{$t_i=\hat{T}_i(\pi')$}
		\EndFor
        \State{$x_i=\Delta x_i+x_i^0$}
        \label{alg:gn.pay0}
		\EndFor
		%\State{Compute parameters independent from report: $(c_{Fmin},c_{Fmax},\hat{\vect{T}}_{min})=\textproc{PaymentParam}()$} \label{alg:gm.payparam}
		%\State{Add base payment: $\vect{x}=\Delta\vect{x}+\textproc{BasePayment}(\hat{\vect{T}}_{min},c_{Fmax})$}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
	\caption{Greedy Allocation}
	\label{alg:ga}
	\begin{algorithmic}[1]
		%\Input Ordered set of riders $\mc{N}$
		%\Output Allocation $\vect{\pi}$
		\Procedure{$\pi=$GreedyAlloc}{$\vect{\gamma},\mc{N}$}
		%\State{$\mc{N}_g=[],\vect{\pi}_{last}=None$}
		\For{$i \in \mc{N}$} \label{alg:ga.iter}
		\State{Compute $\pi_{\leq i}$ by (\ref{eq:gars_notaxi})} \label{alg:ga.solve}
		%\State{Solve $RS^*$ subject to no taxi constraint and keeping $j<i^*$ fixed, and replace $\vect{\pi}_{last}$ with the solution} \label{alg:ga.solve}
		\EndFor
		\State{Return $\pi_{\leq i}$}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


\color{black}

Now we have the following result.

\begin{theorem}
The GARS-NIR mechanism satisfies DSIC, IR, BB and can be computed in polynomial-time.
\label{thm:garsnir}
\end{theorem}

%Note that this result is not trivial but actually quite challenging because the GARS-NIR mechanism has to fulfill the properties independently from the riders’ reports. For example, let’s say a rider makes a detour to share the ride with others. If the rider misreports a high gamma (a higher urgency), the mechanism may let the rider use the vehicle alone without the detour. This can violate DSIC. This can also violate IR of other riders that share the vehicle and cause them to use a taxi instead. The GARS-NIR mechanism solves this issue by computing the set of riders that satisfy IR before receiving their reports, and by keeping the allocation DSIC among the set of riders by preventing manipulation like the example above with the no-taxi constraint.
%One of the challenges of IR is that the mechanism has to guarantee IR before riders report their types. Otherwise, riders can manipulate the allocation by misreporting, thus breaking DSIC. 

Although GARS-NIR is not optimal, also note that no mechanism can simultaneously achieve optimality, DSIC, IR and BB \cite{myerson1983efficient}. Hence obtaining three of these properties is the best one can achieve. \modified{It is also difficult to bound the efficiency of GARS-NIR, because we cannot use the standard bounding technique with naive greedy allocations \cite{nemhauser1978analysis}, for the reason we discussed in Proposition \ref{thm:naivegreedy}.} 
\modified{Determining theoretical efficiency bounds remains an open problem for future work.}


\color{black}



\section{Experimental Results}
\label{sec:exp}

Given that we do not have formal efficiency bounds, we evaluate the mechanisms empirically using simulations using both synthetic and real data. For the former, we generate 
random road networks of 4 degrees maximum and average results over 32 simulations for each setting. For the latter, we use the New York taxi data set \cite{nycdata}. We assume autonomous vehicles for all our experiments.
%randomly generated road networks that are connected with a maximum of 4 degrees. 
%\commenteg{Incomplete: need to mention e.g. that CPLEX was used, and what type of processor+operating system was used to run the experiments on.}
%We tested several cases by chainging parameters $N,K,T,V$ and $\alpha$.
%We use parameters $N=3,K=2,T=4,V=4$ and $\alpha$. 
 %
%meaning that vehicles can move even without anyone being allocated to them. 
%An example of the game is shown in Figure \ref{fig:example}. 
We vary the taxi cost $\alpha$ and choose these loosely based on prices from London taxis. If we normalize the fuel cost to be $\beta=1$, then $\alpha=5$ is considered a moderate value and $\alpha=1$ is cheap. As for the value of time, we set $\gamma_i=\gamma_{max}*i/N$ to simulate heterogeneous riders. $c_{Fub}$ is estimated by sampling solutions of GARS-N with different allocation orders, and multiplying the maximum fuel cost among the solutions with a constant coefficient. \camera{Further details are provided in the extended version.}
%we set the value of use an arithmetic progression of length $N$  from 1 to $\gamma_{max}$ that is in the same order as $i$, simulating a heterogeneous rider population.


%Cost parameter $\alpha$ (wage of taxi drivers) has impact especially on IR. The ratio $\alpha/\beta$ is about 42 according to the cost analysis of taxi company in Switzerland \cite{Bosch2018}. In case of Japan, this number is about 3.8. We think $\alpha=5, \beta=1$ is a moderate setting. We also test an extreme case of $\alpha=0$. 
%\commenteg{These values are too different and not credible. How can Switzerland and Japan be so different? Also strange to use such precise numbers. How did you get these? What value did you set for$\beta$?  These things can never be measured so precisely. The point is to only base these values LOOSELY on some motivation. }

In what follows we first compare the performance of all mechanisms on a small setting to enable comparison with non-scalable mechanisms such as BVCG. We then evaluate the scalability of the greedy mechanism to larger settings. Since GARS-NIR computes all possible ways for a rider to switch  between  vehicles, this turns out to be time consuming computationally. Also, in practice, such switches are often not desirable. Hence, for large settings, we modify \modaaai{the feasible set $\Pi$} of GARS-NIR to allow a rider to use only a single vehicle (sGARS-NIR). This version still satisfies the same properties as GARS-NIR. 

\begin{comment}
\subsection{Cost parameters}
\label{sec:paramexp}

\begin{table}[h]
\centering
\caption{Data for parameter estimation}\smallskip
%\resizebox{0.95\textwidth}{!}{ % If your table exceeds the column or page width, use this command to reduce it slightly
\begin{tabular}{|l|l|}
\hline
Gas price & 124 [p/liter] \\
\hline
Wage of driver & 836 [GBP/week] \\
\hline
Working hour of driver & 50 [h/week] \\
\hline
Taxi speed & 30 [km/h] \\
\hline
Mileage & 11.7 [km/liter]\\
\hline
\end{tabular}
%}
\label{tbl:param}
\end{table}


First, we  choose a realistic value for the cost parameter $\alpha$ (wage of taxi drivers), which has a significant impact on IR. To estimate the value, we use  example data from London, specifically, 
gas price: 124 [p/liter], wage of driver: 836 [GBP/week], working hour of driver: 50 [h/week], taxi speed: 30 [km/h] and mileage: 11.7 [km/liter].
Then, the estimated wage of taxi drivers is $836/50/30*100=55.7$ [p/km] and fuel cost is $124/11.7=10.5$ [p/km]. If we normalize the fuel cost as $\beta=1$, then the normalized wage is $55.7/10.5=5.3$. Thus, we use $\alpha=5$ as a moderate value and contrast this with $\alpha=0$ as an extreme value in experiments. As for $\gamma$, we assume that rider $i$'s type is $\gamma_i=i$, simulating a heterogeneous rider population.
\end{comment}

\begin{comment}
\begin{table}[H]
\centering
\caption{Proposed mechanisms}\smallskip
%\resizebox{0.3\textwidth}{!}{ % If your table exceeds the column or page width, use this command to reduce it slightly
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Mechanism & OPT & DSIC & IR & BB & POLY \\
\hline
VCG & Y & Y & Y & N & Y \\ 
BVCG & N & Y & Y & Y & N \\
Hungarian & N & Y & Y & N & Y \\
GARS-NIR & N & Y & Y & Y & Y \\
\hline
\end{tabular}
%}
\label{tbl:mechs}
\end{table}
\end{comment}


\subsection{Small Setting}
\label{sec:smallexp}

\begin{table}[t]
\centering
%\caption{Characteristics of mechanisms}\smallskip
%\resizebox{0.3\textwidth}{!}{ % If your table exceeds the column or page width, use this command to reduce it slightly
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Mechanism & OPT & DSIC & IR & BB & POLY \\
\hline
VCG & Y & Y & Y & N & Y \\ 
BVCG & N & Y & Y & Y & N \\
Hungarian & N & Y & Y & N & Y \\
GARS-NIR & N & Y & Y & Y & Y \\
\hline
\end{tabular}
%}
\caption{Characteristics of mechanisms.}
\label{tbl:mechs}
\end{table}


\begin{figure}[t]
\centering
\includegraphics[width=1.\columnwidth]{fig/results.pdf}
\caption{Comparison of mechanisms with different taxi costs: \mbox{$\alpha=5$ (top),} $\alpha=1$ (bottom).}
\label{fig:results}
%\vspace{-0.2cm}
\end{figure}

We compare VCG, BVCG, GARS-NIR, the Hungarian mechanism and the outside option
\camera{(Table 1).}
The Hungarian mechanism computes an optimal 1-to-1 matching between riders and vehicles (including taxis) using the Hungarian algorithm, and then applies payments similar to VCG. The mechanism is also DSIC, BB and IR, but does not support multiple riders per vehicle. 
%We compare mechanisms and the outside option.
%In addition to VCG, BVCG, and our greedy mechanism we compare these against the Hungarian mechanism and the outside option. The Hungarian mechanism computes a minimum cost \mbox{1-to-1} matching between riders and vehicles (including taxis) using the Hungarian algorithm. The payments are the marginal social cost (as in VCG). 
For BVCG, a brute force search is used to compute vehicle allocations. 
%Table \ref{tbl:mechs} summarizes these mechanisms.
Figure \ref{fig:results} (top) shows the results for $N=3,K=2,T=4,V=4$ and $\alpha=5$ and the error bars show the 95\% confidence intervals. Here, \emph{social cost} is the \modaaai{ratio of $C_F(\mc{N},\pi)$ over the cost of the optimal allocation.} Furthermore, \emph{IR cost} refers to $-u_i(\pi)/c_i^0$. If this value is above 1, it means that IR is violated. \emph{BB coverage} shows 
$(\sum_{i \in \mc{N}}x_i(\pi))/ c_F(\pi)$.
%the rate of the total payment compared to the fuel cost $c_F$.
A value less than 1 means BB is violated  \camera{(however, a value close to 1 is preferred, as long as it is over 1, meaning that riders are not over paying).}
\modaaai{Share rate shows $\sum_{k \in \mc{K}} T_k/\sum_{i \in \mc{N}} T_i$. A smaller value means ridesharing needs fewers vehicles to cover the trips of riders. }
%the proportion of simulations where individual rationality and budget balance hold. 
%\modaaai{As explained in section ----, sometimes payment is zero in VCG and then BB coverage is infinite. Meanwhile,} 

Here, BVCG is budget balanced without a large increase in social cost (a 6.4\% increase). 
%When VCG violates the BB condition, it 
Meanwhile, VCG recovers only 52\% of the fuel costs on average in payments. However, a disadvantage of BVCG is its computational complexity when using the brute force search. Instead, \modaaai{GARS-NIR (and sGARS-NIR)} can be computed efficiently while satisfying DSIC, IR and BB, and still keeping social cost near optimal (an 8.6\% increase compared to optimal).  Also, it shows that the performance of sGARS-NIR is close to GARS-NIR.
%\modified{As other indicators for a reference, the travel time of GARS-NIR increases 48\% compared to taxi on average. And about 1.23 passengers ride on a vehicle on average.} 
\camera{Although the vehicle-switching behaviors of GARS-NIR are practical in suburban areas, it may not be so practical in urban areas. However, the result shows only $\frac{1}{6}$ of riders switch vehicles. Besides, it is possible to extend the model to introduce a waiting time for switching vehicles, and this can reduce the number of the cases. Also, it is easy to extend the model by mixing GARS-NIR with the version without switching (sGARS-NIR), and letting riders choose if they want to switch or not. 
%Even in this case, the efficiency of allocations is maintained because the riders would suffer from a higher cost when they choose not to switch, by causing fewer options of allocations.
}
%\camera{Although we do not consider the waiting time when riders switch vehicles, the result shows only $\frac{1}{6}$ of riders switch vehicles and so introducing wait times would unlikely have a significant influence on these results.}
In comparison, Figure \ref{fig:results} (bottom) shows the result when the outside option is cheap ($\alpha=1$). In this case, the IR cost comes closer to 1 for all mechanisms because of the incentive to opt out. BB coverage also decreases for some mechanisms because as more riders opt out, there is less opportunity to split the fuel cost. Meanwhile, the increase in social cost is not large in \modaaai{GARS-NIR} (4.5\%) because riders properly opt out \modaaai{if taxi is better}.
\modified{While 1.07 passengers ride on a vehicle on average in case of $\alpha=1$, it is 1.23 passengers in case of $\alpha=5$. This demonstrates that more expensive taxis lead to a higher usage of ridesharing, enabled by GARS-NIR satisfying IR of riders.}
%also performs slightly and only has a 4.5\% increase compared to optimal.

%As for the runtime, BVCG takes 7.4 seconds to compute an allocation, while our greedy method takes only 0.38 seconds. Thus, even in these small settings, it is 19 times faster. Also, since our greedy algorithm computes allocations several times by changing the priority of riders, we can speed up the computation by parallelizing it for each priority case. The main reason we use this small setting in experiments is to compare with non-scalable mechanisms such as BVCG. 

%However, our approach may not yet be sufficiently scalable for very large settings, and this is subject to future investigation.

\begin{comment}
\begin{table*}[t]
\centering
\caption{Experimental results}\smallskip
%\resizebox{0.95\textwidth}{!}{ % If your table exceeds the column or page width, use this command to reduce it slightly
\begin{tabular}{|l|l|}
goodcase & 
badcase \\
\hline
good & 
bad \\ 
\end{tabular}
%}
\label{tbl:result}
\end{table*}
\end{comment}


\subsection{Scalability}
\label{sec:largeexp}

Next, we evaluate the scalability of sGARS-NIR. Since other mechanisms such as BVCG
%and Hungarian 
are not scalable, we do not include them  here. Figure \ref{fig:totalelp} shows the runtime of the mechanism with different $N$ using parallel computation with 16 cores. Since the payment computation consists of independent computations of allocations with different orders of riders, it can be easily parallelized. For other parameters we use $K=N/2, T=15, V=10, \alpha=5, \beta=1$. sGARS-NIR takes less than 14 minutes when $N=40$. 
%If the computation is fully parallelized with more cores, it would finish within 4.5 seconds. 
Figure \ref{fig:runtime}
shows that more than 99\% of the computation
time is spent constructing CPLEX LP objects. \modified{Hence, much of this can be precomputed and addressed with specalised implementation.}
%This is at least in part an implementation issue rather than the algorithm itself.
%For further scalability, we can use the technique to decompose the problem into independent subgames based on the location proximity \cite{xiong2015}.

\color{black}

\begin{figure}[t!]
\centering
\includegraphics[width=1.\columnwidth]{fig/totalelp.pdf}
%\vspace{-0.2cm}
\vspace{-0.2cm}%
\caption{Runtime of sGARS-NIR.}
\label{fig:totalelp}
\vspace{-0.2cm}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=1.\columnwidth]{fig/runtime.pdf}
\vspace{-0.2cm}
\caption{Figure showing a breakdown of the runtime. As can be seen, most of the runtime is spent constructing LP object, instead of solving it.}
\label{fig:runtime}
\vspace{-0.2cm}
\end{figure}
%
\begin{figure}[t!]
\centering
\includegraphics[width=1.\columnwidth]{fig/nycsc.pdf}
\vspace{-0.4cm}
\caption{Performance as the number of riders (N) increases.}
\label{fig:nycsc}
\end{figure}
%
\begin{comment}
First, we measured the computation time of ridesharing problem $RS^*$ in the greedy mechanism with $N=10, K=4,T=11,V=10,\alpha=5$.
%\commenteg{Not clear why Hungarian is not scalable, since it is cubed in terms of computation, and also why VCG is not scalable - we said it was polynomial before for a given value of w!!Needs to be explained} 
Figure \ref{fig:runt} shows the result.
%\commenteg{First you need to tell the reader what the setting is!! You have not said what experiments you have run!} 
It shows that more than 99\% of the computation time is spent  constructing LP objects, not solving the LP. Therefore, although Theorem \ref{thm:poly} shows that the greedy is scalable in theory, the current implementation requires further work to make it scalable in practice. 
%
\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{fig/runtime.pdf}
\caption{Runtime of ridesharing problem $RS^*$}
\label{fig:runt}
\end{figure}

Despite  the issue above, we also evaluate the performance of the greedy mechanism for $N=5,K=4,T=11,V=10$. We can see that, with $\alpha=5$, the IR condition is satisfied in 56\% of the cases, even though the necessary condition (\ref{eq:irn}) is satisfied in all cases. In these cases, riders pay on average about 19\% more than the outside option. With $\alpha=0$, 8\% of the cases satisfy the necessary condition of IR in (\ref{eq:irn}) and no cases satisfy IR. Riders pay on average 74\% more than the outside option. These results are worse than the ones in smaller settings in the previous section. One of the reasons is that the impact of inefficient detours caused by the no-taxi constraint becomes larger when the size of road network increases. In all cases, BB is satisfied. 
\end{comment}

\subsection{Experiments with Real-world Data}
\label{sec:realexp}

In addition to using synthetic data, we also conduct experiments using the New York taxi data set \cite{nycdata}. We analyse the traffic demands in the central Manhattan area, which consists of 19 zones.
%64 zones. 
A single trip data point includes the origin zone, the destination zone, departure and arrival time. We randomly generate trip demands with the trip distribution from February 2019. All riders are assumed to be picked up and dropped off at the center of their zones. We set $K=20, T=15, V=19, \alpha=5, \beta=1$ and vary $N$. Figure \ref{fig:nycsc} shows the ratio of social cost compared to the taxi cost, IR cost, BB coverage and share rate of sGARS-NIR. 
\camera{The share rate is improved as $N$ increases since this increases the chance of sharing vehicles. However, with $K$ fixed, increasing $N$ causes a lack of vehicles and thus an increase in the IR cost and the social cost. This can be solved by providing an appropriate number of vehicles. The BB coverage shows over payment of riders with large $N$, but they still save compared to taking a taxi.}
%All measurements improved as the problem size increases since this increases the chance of sharing vehicles.


\section{Conclusions}
\label{sec:conclusions}
%To realise an efficient, safe and convenient ridesharing system with upcoming autonomous vehicles, a practical mechanism is required that allocates vehicles effectively and promotes the usage of riders by giving them an incentive.
We propose a flexible ridesharing model that includes autonomous vehicles.
%the ability of riders to  switch between vehicles. 
The goal is to \modified{find allocation and payment mechanisms which are dominant-strategy incentive compatible,} budget balanced, individually rational, can be computed in polynomial time and achieve high social welfare. To this end, we \modified{show that both the VCG and naive greedy mechanisms do not meet these requirements.} We then present a  characterisation for monotone greedy allocations and  use this  to develop a novel greedy mechanism which satisfies all of the desirable properties. In addition, through numerical simulations we show that \modified{our} monotone greedy mechanism achieves close to optimal allocations. 
%when assuming realistic taxi costs. 

Future directions include \modaaai{envy-free mechanisms and} improving the implementation of the algorithm so it scales to even larger settings, as well as providing theoretical performance bounds for our  greedy approach. %This can be achieved by decomposing the problem into independent subgames based on the location proximity similar to, for example, \cite{xiong2015}.

%\newpage

\begin{comment}

\begin{appendices}

\section{}


%\subsection{Efficient Computation of Rideshring Problems as a Linear Program}
%\label{sec:lp}

Here we show an efficient algorithm to solve the ridesharing problem. As in the traditional studies of DARP \cite{Laporte2007}, we represent the solution with binary variables. Let $x_{i,t,e}^p=1$ if rider $i$ moves on edge $e$ at time $t$ and $x_{i,t,e}^p=0$ otherwise. Similarly, $x_{k,t,e}^c=1$ when vehicle $k$ moves on edge $e$ at time $t$. $\vect{x}$ denotes the vector of all variables. Then the ridesharing problem $RS$ is formulated as the following integer linear program (ILP).

\begin{equation}
    \left.
    \begin{array}{ll}
    \underset{\substack{\vect{x}}}{\min}&\underset{\substack{i \in \mc{N}_g}}{\sum}\underset{\substack{t \in \mc{T}}}{\sum}\underset{\substack{e \in \mc{E}}}{\sum}\gamma_i x_{i,t,e}^p l_{e,i}
    +\underset{\substack{k \in \mc{K}}}{\sum}\underset{\substack{t \in \mc{T}}}{\sum}\underset{\substack{e \in \mc{E}}}{\sum}\beta x_{k,t,e}^c l_e \\
    s.t.&
    \end{array}
    \right.
	\label{eq:mipobj}
\end{equation}

    \begin{equation}
    x_{i,t,e}^p,x_{k,t,e}^c\in \{0,1\}, ~\forall i \in \mc{N}_g,k \in \mc{K},t \in \mc{T},e \in \mc{E}
	\label{eq:mipbin}
    \end{equation}

    \begin{equation}
    \left.
    \begin{array}{l}
    \underset{\substack{e \in \mc{E}}}{\sum}x_{i,t,e}^p=1, ~\forall i \in \mc{N}_g,t \in \mc{T} \\
    \underset{\substack{e \in \mc{E}}}{\sum}x_{k,t,e}^c=1, ~\forall k \in \mc{K},t \in \mc{T}    
    \end{array}
    \right.
	\label{eq:mipexcl}
    \end{equation}

    \begin{equation}
    \left.
    \begin{array}{l}
    \underset{\substack{e = (v_k^0,*) }}{\sum}x_{k,0,e}=1, ~\forall k \in \mc{K} \\
    \underset{\substack{e = (v_i^0,*) }}{\sum}x_{i,0,e}=1, ~\forall i \in \mc{N}_g  
    \end{array}
    \right.
	\label{eq:mipo}
    \end{equation}

    \begin{equation}
    \underset{\substack{e = (*,v_i^T)}}{\sum}x_{i,t,e}^p=1, ~\forall i \in \mc{N}_g
	\label{eq:mipd}
    \end{equation}
    
    \begin{equation}
    x_{i,t,e}^p\leq \underset{\substack{k\in \mc{K}}}{\sum}x_{k,t,e}^c, ~\forall i \in \mc{N}_g,t \in \mc{T},e=(o,d\not=o) \in \mc{E}
	\label{eq:mipnotaxi}
    \end{equation}

    \begin{equation}
    \underset{\substack{i\in \mc{N}_g}}{\sum}x_{i,t,e}^p\leq w\underset{\substack{k\in \mc{K}}}{\sum}x_{k,t,e}^c, ~\forall t \in \mc{T},e=(o,d\not=o)\in \mc{E}
	\label{eq:mipcap}
    \end{equation}

    \begin{equation}
    \left.
    \begin{array}{l}
    \underset{\substack{e = (*,v) }}{\sum}x_{i,t,e}^p=\underset{\substack{e = (v,*) }}{\sum}x_{i,t+1,e}, ~\forall i \in \mc{N}_g,t \in \mc{T},v \in \mc{V} \\
    \underset{\substack{e = (*,v) }}{\sum}x_{k,t,e}^c=\underset{\substack{e = (v,*) }}{\sum}x_{k,t+1,e}, ~\forall k \in \mc{K},t \in \mc{T},v \in \mc{V}    
    \end{array}
    \right.
	\label{eq:mipconn}
    \end{equation}
    
    \begin{equation}
    x_{j,t,e}=1, e={\rm edge}(r_j^p,t),~\forall t\in \mc{T},j<i^* \in \mc{N}
    %x_{j,t,e}=1, ~\forall (e,t)\in {\rm each}(r_j^p),j<i^* \in \mc{N}
	\label{eq:mipgrd}
    \end{equation}

(\ref{eq:mipobj}) shows the objective function $C_F(\mc{N},\pi)$. $l_{e,i}$ denotes length of edge $e=(O,D)$, but if $O=D$ and $D\not= D_i$ then $l_{e,i}=1$. This is a trick to represent waiting costs of riders.  (\ref{eq:mipbin}) represents a binary constraint. (\ref{eq:mipexcl}) means that riders and vehicles can choose only one edge at a time. (\ref{eq:mipo}) represents the origin of riders and vehicles. (\ref{eq:mipd}) represents the destinations. (\ref{eq:mipnotaxi}) shows one of the assumption of the mechanism, that no riders use taxi. (\ref{eq:mipcap}) represents the capacity of the vehicles. (\ref{eq:mipconn}) represents the all successive moves are connected. (\ref{eq:mipgrd}) represents the solutions of riders that are already computed in former iteration of the greedy mechanism. 

For the ridesharing problems $RS_T$ and $RS_F$ in Algorithm 3, we switch the objective function to (\ref{eq:mipobjtmin}) and (\ref{eq:mipobjcf}), respectively.

\begin{equation}
    \underset{\substack{\vect{x}}}{\min}\underset{\substack{i \in \mc{N}_g}}{\sum}\underset{\substack{t \in \mc{T}}}{\sum}\underset{\substack{e \in \mc{E}}}{\sum}x_{i,t,e}^pl_e
	\label{eq:mipobjtmin}
\end{equation}

\begin{equation}
    \underset{\substack{\vect{x}}}{\min}\underset{\substack{k \in \mc{K}}}{\sum}\underset{\substack{t \in \mc{T}}}{\sum}\underset{\substack{e \in \mc{E}}}{\sum}x_{k,t,e}^cl_e
	\label{eq:mipobjcf}
\end{equation}


Henceforth we refer to  these ridesharing problems formulated in ILP  as RSILP. Solving RSILP, we obtain routes of riders and vehicles, but the assignment of vehicles to riders is not computed yet. However, any assignments can be a solution for each set of riders and vehicles that share a same edge at the same timing. This assignment can be done easily with existing matching algorithms, such as the Hungarian algorithm. With an assumption of fixed capacity, RSILP can be efficiently computed according to Theorem 2. Here is the proof.

\begin{proof}[Proof of Theorem 2]
The constraints of RSILP is denoted by $A\vect{x}\leq \vect{b}$ as a matrix form. If all the elements of $A$ belong to $\{-1,0,1\}$ and $\vect{b}$ is integer, the solutions of relaxed linear program (LP) are integers and coincide with the solutions of the original ILP \cite{wolsey1999integer}. The only elements that are not in $\{-1,0,1\}$ come from capacity $w$ in constraint (\ref{eq:mipcap}).
Now we consider a conversion of the problem by splitting a vehicle of capacity $w$ into $w$ vehicles of capacity 1. If those vehicles move on exactly same route as the original vehicle, it gives the equivalent problem to the original one. Since capacity of vehicles is 1 in the converted problem, now all elements of $A$ belong to $\{-1,0,1\}$. Then the problem can be relaxed into LP, by replacing constraint (\ref{eq:mipbin}) with the following constraint.

\begin{equation}
    x_{i,t,e}^p,x_{k,t,e}^c\in [0,1], \forall i,k,t,e
	\label{eq:miprelax}
\end{equation}

The solution of this LP is an exact solution of the original RSILP. 
Since the number of variables and the numberof constraints are polynomial in the size of the problem $N,K,T,V,w$, the LP can be solved in pseudo polynomial time \cite{JohnsonDavidS.1979}. If we assume that $w$ is fixed, the LP can be solved in polynomial time.
\end{proof}

\end{appendices}
\end{comment}



==> SOTON IJCAI2021/ethics.tex <==
\section*{Ethical Impact}

Our work has positive ethical impacts on society. First, our mechanism provides a fair ridesharing service in the sense that people get compensated for their detour. Second, the incentive compatibility of our mechanism maximizes the utility of individuals. Third, our ridesharing mechanism can benefit society and the environment by meeting more traffic demand with fewer vehicles than existing taxi services or privately-owned vehicles. A possible negative impact is that people might perceive the mechanism as unfair because the payments for a given service may differ depending on the other participants. We could address this by looking into envy-free mechanisms in  future work.

==> SOTON IJCAI2021/include.tex <==
%\usepackage[noadjust]{cite}
%\usepackage{biblatex}
%\usepackage[a-1b]{pdfx} 
\usepackage{amssymb,amsfonts}
\usepackage{textcomp}
\usepackage{xcolor}
%\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\usepackage{comment}
\usepackage{url}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
%\usepackage{babel}
\usepackage{blindtext}
\usepackage{pdfpages}

%\usepackage{times}
%\usepackage[numbers]{natbib}
%\PassOptionsToPackage{square,numbers}{natbib}
%\usepackage[title,titletoc]{appendix}
%\usepackage[dvipdfmx]{color}
%\usepackage[dvipdfmx]{graphicx}
\usepackage{here}
\usepackage{xcolor}
\usepackage{fancyhdr}
%\usepackage{ulem}
\excludecomment{hdn}
%\usepackage{xr}
%\externaldocument{body}
\usepackage[title,titletoc]{appendix}

\usepackage{ascmac}
\usepackage{bm,enumerate,amsmath,amssymb,amsthm}
%\theoremstyle{break}
\newtheoremstyle{assumption}% name
  {\topsep}% space above
  {\topsep}% space below
  {}% body font
  {1em}% indent amount
  {\itshape}% theorem head font
  {}% punctuation after theorem head
  {.5em}% space after theorem head
  {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}% theorem head spec
\theoremstyle{assumption}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{observation}{Observation}
\newtheorem{minortheorem}{Proposition}

\usepackage[noend]{algpseudocode}
\algnewcommand\Input{\item[{\textbf{Input:}}]}
\algnewcommand\Output{\item[{\textbf{Output:}}]}
\algrenewcommand\algorithmicdo{}
\algnewcommand\algorithmicto{\textbf{to}}
\algnewcommand\algorithmicbreak{\textbf{break}}
\algdef{SE}[FOR]{ForTo}{EndFor}[2]{\algorithmicfor\ #1\ \algorithmicto\ #2\ \algorithmicdo}{\algorithmicend\ \algorithmicfor}%
\algtext*{EndFor}
\let\oldReturn\Return
\renewcommand{\Return}{\State\oldReturn}
\renewcommand{\algorithmiccomment}[1]{{\# #1}}
\newcommand{\Break}{\State \algorithmicbreak}

\def \vect#1{\mbox{\boldmath $#1$}}
\newcommand{\mc}{\mathcal}
\newcommand{\capup}{\vspace{-3truemm}}
\newcommand{\argmax}{\mathop{\rm argmax~}\limits}
\newcommand{\argmin}{\mathop{\rm argmin~}\limits}
\newcommand{\ison}{{\rm ~is~on~}}
\newcommand{\rif}{{\rm ~~if~}}
\newcommand{\succeed}{{\rm ~succeeds~}}
\newcommand{\precede}{{\rm ~precedes~}}
\newcommand{\term}{{\rm ~terminates~}}
\newcommand{\agree}{{\rm ~agrees~with~}}
\newcommand{\incl}{{\rm ~includes~}}
\newcommand{\inn}{{\rm ~in~}}
\newcommand{\strat}{\rule{0pt}{2ex}}
\newcommand{\red}{\textcolor{red}}
\newcommand{\impact}{{\rm Impact}}
\newcommand{\leaf}{{\rm leaf}}
\newcommand{\pt}{{\rm path}}
\newcommand{\shortest}{{\rm shortestpath}}
\newcommand{\argsort}{{\rm argsort}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

%\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\newcommand{\newcolor}{black}

\newcommand{\memo}[1]{\textcolor{red}{#1}}

\newcommand{\commentti}[1]{\textcolor{blue}{\textbf{Tatsuya Says: #1}}}
\newcommand{\modaaai}[1]{\textcolor{black}{#1}}
\newcommand{\modified}[1]{\textcolor{black}{#1}}
%\newcommand{\extref}[1]{\textcolor{blue}{Equation #1 in the paper}}
\newcommand{\extref}[1]{Equation #1 in the paper}

\def\arxiv{1}
\newcommand{\cameracolor}{black}


\if\arxiv0
\newcommand{\camera}[1]{\textcolor{\cameracolor}{#1}}
\else
\newcommand{\camera}[1]{\textcolor{\cameracolor}{#1}}
\fi
\newcommand{\urlblue}[1]{\textcolor{blue}{#1}}




==> SOTON IJCAI2021/poster.tex <==
\begin{itemize}
    \item Both riders 1\&2 want to go to B.
    \item Rider $i$ report “value of time” $\gamma_i$.
    \item Mechanism: allocation $\pi$ \& payment $x_i(\pi)$
    \item Rider cost: $c_i(\pi)$=travel time$*\gamma_i$
    \item Rider utility: $u_i(\pi)=-c_i(\pi)-x_i(\pi)$
    \item Discount price if rider 1 detours for pickup.
\end{itemize}

\begin{equation}
 \left.
 \begin{array}{ll}
 &\underset{\substack{(\pi,x)\in \Pi\times \mc{X}}}{\min}\sum_{i \in \mc{N}}c_i(\pi)+c_F(\pi)\\
 \\
 s.t.&
u_i(\pi)\ge-c_i^0,\\
\\
&\sum_{i \in \mc{N}}x_i(\pi)\ge c_F(\pi), \\
\\
&u_i(\pi(\gamma_i,\gamma_{-i}))\ge u_i(\pi(\gamma_i',\gamma_{-i})). 
%~\forall \gamma_i' \in \Gamma,  ~\forall i \in  \mc{N}, \forall \gamma_{-i} \in \Gamma^{N-1},
\\
\\
 \end{array}
 \right.
\end{equation}

Social optimum (SO): \\System tries to minimize rider cost $+$ fuel cost.


==> SOTON IJCAI2021/supplementalbody.tex <==
\setcounter{secnumdepth}{0} %May be changed to 1 or 2 if section numbers are desired.

% The file aaai20.sty is the style file for AAAI Press 
% proceedings, working notes, and technical reports.
%
% command to correct it. You may not alter the value below 2.5 in
\title{Scalable, Truthful and Budget Balanced Ridesharing Mechanisms \\ (supplemental material)}

\author{Paper ID 8002}


\begin{appendices}

\section{Appendix A: NP-hardness of the Ridesharing Problem}

\label{sec:lp}
\color{\newcolor}
We show the following negative result on the computational complexity of the RS problem.

\setcounter{minortheorem}{4}
\begin{minortheorem}
    Finding an optimal solution of the RS problem is NP-hard.
	\label{thm:NPh}
\end{minortheorem}

\begin{proof}
Consider the NP-hard Travelling Salesman Problem (TSP), i.e., the problem to find the shortest cycle in a graph that visits all vertices. Any TSP can be reduced to a special case of the ridesharing problem where: 
\begin{itemize}
    \item The road network, $\mc{G}=(\mc{V},\mc{E})$,  is the same network as in the TSP. There is one rider on every vertex. 
    \item There is only one vehicle $k$, and its capacity is $w=N$. It can be placed on any vertex of the road network.
    \item The taxi cost is $\alpha>\sum_{e\in \mc{E}}1$, which is too expensive for riders to use.
    \item The vehicle is autonomous.
    \item Riders' destination is equal to the origin of the vehicle as $D_i^p=O_k^c,~\forall i\in\mc{N}$.
    \item $\gamma_i=0,~\forall i\in\mc{N}$,  $\beta=1$ and $T = |\mc{E}|$.
\end{itemize}

As the only cost incurred in this version of the RS problem is the fuel cost, the vehicle will choose the shortest cycle in the graph to pick up all riders. This is the same solution as the original TSP problem. Since any TSP can be reduced to an RS problem in polynomial time, the RS problem is also NP-hard.
\end{proof}


\section{Appendix B: Complete Proofs of Theorems}
\label{sec:proof}


\subsection{Proof of Proposition 2}

\color{\newcolor}

\begin{proof}
The BVCG mechanism can be seen as a VCG mechanism with an additional player 0 added. In more detail, consider an allocation problem among riders (players $1,\ldots,N$) and a ridesharing system (player $0$) who does not move and has no need for cars. The cost function of the system (i.e., player 0) is $c_F(\pi)+c_I(\pi)$. We then use the VCG mechanism for this problem. Since BVCG is an instance of VCG, DSIC and IR of all riders are trivially satisfied. Note that we are not concerned about DSIC and IR of the system player and can ignore its payment. A similar approach was used by \cite{Jehiel2006} for a different setting. 
%\commenteg{To me there seems to be something missing: we also need to show/state that the other agents cannot influence the cost function of player 0, otherwise this would indirectly affect their payment}

%\modaaai{Proofs are omitted due to the limited space. Briefly, this is because BVCG mechanism is a subset of VCG.}

\color{black}

%\ref{thm:bb}
\modified{Now we prove the BB property by assuming autonomous vehicles.}
We first obtain the following lemma, which shows the relationship between the fuel cost and the imaginary cost for a given allocation.

\setcounter{lemma}{4}
\begin{lemma}
	$c_F(\vect{\pi}) \leq c_I(\vect{\pi}) \leq N*c_F(\vect{\pi})$
	\label{thm:imaginary}
\end{lemma}

Intuitively this is because, if riders use the same vehicle, everyone's individual imaginary cost can be equal to $c_F$ in the worst case.

Moreover, the following lemma describes the change in social cost when a rider is removed from the mechanism.

\begin{lemma}
    Assuming autonomous vehicles, \\
	$C_I(-i,\vect{\pi})-c_I^i(\vect{\pi}) \geq C_I(-i,\vect{\pi}_{-i})$.
	\label{thm:absence}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{thm:absence}]
Let $\vect{\pi}\setminus i$ denote an allocation for the set of riders $-i$, which is completely the same as $\vect{\pi}$, with the same set of vehicles and the same routes. The only difference is the absence of rider $i$. Such a route is still feasible because of the autonomous vehicles assumption (where vehicles can move without riders). 

Because of the absence of $i$ in $\vect{\pi}\setminus i$, the system social cost loses the cost related to $i$, which is,

\begin{equation}
 \left.
 \begin{array}{l}
 C_I(-i,\vect{\pi}\setminus i)\\
 =C_I(\mc{N},\vect{\pi})-c_i(\vect{\pi})-c_I^i(\vect{\pi}) \\
 =C_I(-i,\vect{\pi})-c_I^i(\vect{\pi}).
 \end{array}
 \right.
\end{equation}
 
Although $\vect{\pi}\setminus i$ is feasible, it is not necessarily optimal. Due to the optimality of the allocation for $-i$, we have that:
 
\begin{equation}
C_I(-i,\vect{\pi}\setminus i) \geq C_I(-i,\vect{\pi}_{-i})
\end{equation}
 
Then the lemma follows.
\end{proof}


To apply Lemma \ref{thm:absence}, we start from the following term
\begin{equation}
x_i-c_I^i(\vect{\pi})= C_I(-i,\vect{\pi})-C_I(-i,\vect{\pi}_{-i})-c_I^i(\vect{\pi}).
\end{equation}

By Lemma \ref{thm:absence}, this is larger than 0 and then $x_i\geq c_I^i(\vect{\pi})$.

Then, by summing up for all riders, $\sum_{i \in \mc{N}}x_i\geq \sum_{i \in \mc{N}}c_I^i(\vect{\pi})=c_I(\vect{\pi})$. Then by Lemma \ref{thm:imaginary}, $\sum_{i \in \mc{N}}x_i\geq c_F(\vect{\pi})$. \modified{This completes the proof of the proposition.}
\end{proof}

\subsection{Proof of Theorem 1}

\color{\newcolor}
\begin{proof}
First we prove it is a sufficient condition. Assume  \extref{7}. If $\gamma_i \leq \gamma_k \leq \gamma_i'$, reporting $\gamma_i$ can only delay the allocation of $i$ compared to reporting $\gamma_i'$. With slight abuse of notation, let $\Pi_{\leq i}(\gamma)$ denote the set of possible allocations when reporting $\gamma$.  Then, $\Pi_{\leq i}(\gamma_i) \subseteq \Pi_{\leq k}(\gamma_k) \subseteq \Pi_{\leq i}(\gamma_i')$.
%, since $\Pi^i(\gamma_i)$ has more constraints in (\ref{eq:greedyfeas}) than $\Pi^i(\gamma_i')$. 
Then,
$J(\pi_{\leq i}(\gamma_i))\geq J(\pi_{\leq i}(\gamma_i'))$.
Then, because of \extref{7}, 
$V_i[\pi_{\leq i}(\gamma_i)]\leq V_i[\pi_{\leq i}(\gamma_i')]$, and then $V_i[\pi(\gamma_i)]\leq V_i[\pi(\gamma_i')]$.
This proves it is a sufficient condition.

Next, we prove it is also a necessary condition. Assume  \extref{5}.
We will prove this by contradiction, first assuming the negation of \extref{7}, which is
\begin{equation}
\left.
\begin{array}{l}
    J(\pi_{\leq i}(\gamma_a))\leq J(\pi_{\leq i}(\gamma_b))\wedge \\
    V_i[\pi_{\leq i}(\gamma_a)]< V_i[\pi_{\leq i}(\gamma_b)],
    \exists \gamma_a, \gamma_b, i \in \mc{N}.
    \label{eq:neg}
\end{array}
\right.
\end{equation}

The first inequality means $\gamma_b \leq \gamma_a$, as inferred above.
Meanwhile, $\gamma_b \leq \gamma_a$ and monotonicity (\extref{5}) give
    $V_i[\pi_{\leq i}(\gamma_a)]\geq V_i[\pi_{\leq i}(\gamma_b)]$,
which contradicts the second inequality in Equation \ref{eq:neg}.
This proves the necessary condition.
\end{proof}


\subsection{Proof of Lemma 1}

\begin{proof}[Proof of Lemma 1]
    %~\\
    Let $\gamma_a, \gamma_b$ be $i$'s reports and $\gamma_j > \gamma_a \geq \gamma_b$. Since the GARS-N is a GADC, then
    
    \begin{equation}
    J(\pi_{\leq i}(\gamma_a))\leq J(\pi_{\leq i}(\gamma_b)).
    \end{equation}
    
    Meanwhile, the constraints of %(\ref{eq:greedyfeasrs}) 
\extref{8}
    does not allow $i$ to change the allocations and costs of other riders. Then,
    
    \begin{equation}
    \left.
    \begin{array}{l}
    \pi_{\leq i}=\underset{\substack{\pi \in\Pi_{\leq i}}}{\argmin}J(\pi)=\underset{\substack{\pi \in\Pi_{\leq i}}}{\argmin}~c_i(\pi).
    \end{array}
    \right.
    \end{equation}
    And then,
    $c_i(\pi_{\leq i}(\gamma_a)) \leq c_i(\pi_{\leq i}(\gamma_b))$. Since the riders later than $i$ cannot change $c_j(\pi_{\leq i})$ either, $c_i(\pi(\gamma_a)) \leq c_i(\pi(\gamma_b))$. Because of the no taxi constraint, $i$ uses ridesharing and then $T_i$ is proportional to $c_i$. Then 
    \begin{equation}
    T_i(\pi(\gamma_a)) \leq T_i(\pi(\gamma_b)).
    \label{eq:gars_alloc}
    \end{equation}

    Since the amount of the  allocation is the negative travel time as $V_i=-T_i$, we have proved 
    %(\ref{eq:consist})
    \extref{7}. This is equivalent to monotonicity according to Theorem 1.
    %\ref{thm:nsmono}
    Note that, if $i$ could take a taxi to reduce $T_i$, then (\ref{eq:gars_alloc}) could be violated since a taxi follows the shortest path.
\end{proof}

\color{black}

\subsection{Proof of Lemma 2}
%\ref{thm:garsn_dsic}
\begin{proof}
First, we prove that the payment scheme %in \textproc{GreedyMechanism}
is a necessary condition of incentive compatibility. From the definition of incentive compatibility,
\begin{equation}
 \left.
 \begin{array}{ll}
&-\hat{c}_i(\gamma_i,\gamma_{-i})-x_i(\gamma_i,\gamma_{-i}) \geq -\hat{c}_i(\gamma_i',\gamma_{-i})-x_i(\gamma_i',\gamma_{-i}) \\
\therefore &(\alpha+\beta)T_i^0-\hat{T}_i(\gamma_i,\gamma_{-i})\gamma_i-x_i(\gamma_i,\gamma_{-i}) \\
&\geq (\alpha+\beta)T_i^0-\hat{T}_i(\gamma_i',\gamma_{-i})\gamma_i-x_i(\gamma_i',\gamma_{-i}) \\
\therefore& [\hat{T}_i(\gamma_i',\gamma_{-i})-\hat{T}_i(\gamma_i,\gamma_{-i})]\gamma_i \geq x_i(\gamma_i,\gamma_{-i})-x_i(\gamma_i',\gamma_{-i})
 \end{array}
 \right.
\end{equation}

Let $0<y<z$. Then,
%\begin{equation}
$[\hat{T}_i(z)-\hat{T}_i(y)]y \geq x_i(y)-x_i(z)$ 
%\end{equation}
and also,
%\begin{equation}
$[\hat{T}_i(y)-\hat{T}_i(z)]z \geq x_i(z)-x_i(y)$. 
%\end{equation}
Then,
%\begin{equation}
$[\hat{T}_i(z)-\hat{T}_i(y)]y \geq x_i(y)-x_i(z) \geq [\hat{T}_i(z)-\hat{T}_i(y)]z$. 
%\end{equation}
Then, when $y\to z$ at a jumping point $z$,
%\begin{equation}
$-\Delta\hat{T}_i(z)z=\Delta x_i(z)$.
%\end{equation}
Then, the incentive compatible payment must be

\begin{equation}
x_i(\gamma_i,\gamma_{-i})=-\underset{\substack{j \in {\rm jumps} \\ z_j \leq \gamma_i}}{\sum}z_j\Delta \hat{T}_i(z_j,\gamma_{-i}).
\label{eq:monopay}
\end{equation}

The payment 
%computed in \textproc{GreedyMechanism} 
satisfies this property. Next, we prove the payment is also a sufficient condition. This payment results in incentive compatibility when the allocation is monotone as in the Figure  \ref{fig:gic}. In the figure, $\gamma_i$ is the true type of $i$ and $\hat{\gamma}_i$ is reported value. Then the cost of $i$ is the area shown in gray and the payment is the area in black. Then the utility is maximized when $i$ reports its type honestly.
%The lower side simplifies the upper side by canceling out the blue area. 
\end{proof}

\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{fig/payment.pdf}
\caption{Incentive compatibility with monotone allocation \\
(a) true bidding, (b) over bidding and (c) under bidding}
\label{fig:gic}
\end{figure}

\subsection{Proof of Lemma 3}
%\ref{thm:gbb}
\begin{proof}
Since the base payment $x_i^0$ is computed by splitting $c_{Fub}$ and $x_i\geq x_i^0$,
%computation \textproc{BasePayment}, and since $\Delta \vect{x}\geq \vect{0}$,
\begin{equation}
\underset{\substack{i \in \mc{N}}}{\sum}x_i \geq \underset{\substack{i \in \mc{N}}}{\sum}x_i^0 = c_{Fub} \geq c_{F}.
\label{eq:gbbp}
\end{equation}
\end{proof}

\subsection{Proof of Lemma 4}
%\ref{thm:irs}
\begin{proof}
\begin{equation}
\left.
\begin{array}{l}
[(\alpha+\beta)T_i^0-x_i^0]/\gamma_{max}\geq \hat{T}_i(\vect{\pi}(0))\\
\therefore (\alpha+\beta)T_i^0\geq \gamma_{max}\hat{T}_i(\vect{\pi}(0))+x_i^0\geq \gamma_i\hat{T}_i(\vect{\pi}(0))+x_i^0\\
\therefore (\alpha+\beta)T_i^0-\gamma_i\hat{T}_i(\vect{\pi})\geq  \gamma_i[\hat{T}_i(\vect{\pi}(0))-\hat{T}_i(\vect{\pi})]+x_i^0 \geq x_i(\vect{\pi})\\
\therefore (\alpha+\beta+\gamma_i)T_i^0\geq \gamma_iT_i(\vect{\pi})+x_i(\vect{\pi})\\
\therefore c_i^0\geq c_i(\vect{\pi})+x_i(\vect{\pi})\\
\end{array}
\right.
\end{equation}
\end{proof}

\section{Appendix C: Details of Experiments}
\label{sec:expdetail}

\begin{itemize}
    \item We call numpy.random.seed(1) at the beginning of the main code. 
    \item We use CPLEX 12.7.1, Python 2.7.16, Red Hat Enterprise Linux Server release 6.10 and Intel Xeon CPU E5-2670 (2.60 GHz) with 8 cores, 132 GB memory to run the experiments.
    \item We estimate a realistic value for the cost parameter ${\bf \alpha}$ (wage of taxi drivers), with data from London taxis \cite{londonspeed,londonwage}. Specifically, fuel price: 124 [p/liter], wage of driver: 836 [GBP/week], working hour of driver: 50 [h/week], taxi speed: 30 [km/h] and mileage: 11.7 [km/liter]. Then, the estimated wage of taxi drivers is
    ${\bf 836/50/30*100=55.7}$ [p/km] and fuel cost is ${\bf 124/11.7=10.5}$ [p/km]. If we normalize the fuel cost as ${\bf \beta=1}$, then the normalized wage is ${\bf 55.7/10.5=5.3}$. Thus, we use ${\bf \alpha=5}$ as a moderate value.
\end{itemize}

\color{\cameracolor}
\begin{algorithm}                      
	\caption{Payment Parameter}
	\label{alg:pp}
	\begin{algorithmic}[1]
		\Procedure{$c_{Fub}=$PaymentParam}{}
	    \State{$c_{Fub}=0$}
		\For{$i \in \mc{N}$} \label{alg:pp.dev1}
		\For{$order_i \in [0,\ldots,N]$}
		\For{$j \in -i$}
		\For{$order_j \in [0,\ldots,N]$}
    	\State{$\mc{N}'=\mc{N},\vect{\gamma}'=\vect{\gamma}$}
    	\State{$k=\mc{N}[order_i]$}
		\State{$\mc{N}'.{\rm pop}(\mc{N}.index(i))$}
		\State{$\mc{N}'.{\rm insert}(order_i,i)$}
		\label{alg:pp.movei}
		\State{$\gamma_i'=\gamma_k$}
    	\State{$k=\mc{N}[order_j]$}
		\State{$\mc{N}'.{\rm pop}(\mc{N}.index(j))$}
		\State{$\mc{N}'.{\rm insert}(order_j,j)$}
		\label{alg:pp.movej}
		\State{$\gamma_j'=\gamma_k$}
		\label{alg:pp.dev2}

    	\State{$\pi=\textproc{GreedyAlloc}(\vect{\gamma}',\mc{N}')$} \label{alg:pp.alloc}
    		\If{$c_{Fub} < c_F(\pi)$}
    		\State{$c_{Fub} = c_F(\pi)$} \label{alg:pp.cfmax}
    		\EndIf
		\EndFor
		\EndFor
		\EndFor
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}                      
	\caption{Base Payment}
	\label{alg:bp}
	\begin{algorithmic}[1]
		\Procedure{$\vect{x}^0=$BasePayment}{$\hat{\vect{T}}_{min},c_{Fub}$}
		\State{Compute loss: $\Delta \vect{T}=\vect{T}^0-\hat{\vect{T}}_{min}$} \label{alg:bp.t}
		\State{Normalization: $\Delta \vect{T}=\Delta \vect{T}-\min(\Delta \vect{T})$} \label{alg:bp.nt}
		\If{$\sum(\Delta \vect{T})==0$}
		    \State{$x_i^0=c_{Fub}/N, ~\forall i \in \mc{N}$}
		\Else
		    \State{$k=c_{Fub}/\sum(\Delta \vect{T})$} \label{alg:bp.coef}
		    \State{$x_i^0=k\Delta T_i,~\forall i \in \mc{N}$} \label{alg:bp.prop}
		\EndIf
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


The \textproc{PaymentParam} function (Algorithm \ref{alg:pp}) shows a heuristics to estimate the upper bound of $c_F$.
It searches pairs of deviations of every two riders (line \ref{alg:pp.dev1}-\ref{alg:pp.dev2}) and computes allocations (line \ref{alg:pp.alloc}) to find the upper bound of the fuel cost $c_{Fub}$ (line \ref{alg:pp.cfmax}). 
%Since those parameters are independent from the reports $\vect{\gamma}$, the function \textproc{BasePayment} (Algorithm \ref{alg:bp}) does not break incentive compatibility brought by the monotone allocation. 
The function \textproc{BasePayment} (Algorithm \ref{alg:bp}) shows how to compute the base payment $\vect{x}^0$.
%by splitting $c_{Fub}$ among riders. 
Riders with longer trips and less waiting time pay more. For this purpose, it computes the normalized travel time (line \ref{alg:bp.t},\ref{alg:bp.nt}) and makes the base payment proportional to it (line \ref{alg:bp.coef},\ref{alg:bp.prop}).


\begin{comment}
\section{Appendix D: Reproducibility Checklist}
\label{sec:checklist}

This paper:

\begin{itemize}
    \item clearly states what claims are being investigated (yes)
    \item explains how the results substantiate the claims (yes)
    \item explicitly identifies limitations or technical assumptions  (yes)
    \item includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
\end{itemize}

\subsection{Does this paper make theoretical claims? (yes) }

If yes, please complete the list below. 

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes)
    \item All novel claims are stated formally (e.g., in theorem statements). (yes)
    \item Proofs of all novel claims are included and complete. (yes)
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes)
    \item Appropriate citations to theoretical tools used are given. (yes)
\end{itemize}


\subsection{Does this paper rely on one or more data sets? (yes)} 

If yes, please complete the list below. 

\begin{itemize}
    \item All novel datasets introduced in this paper are described in detail in a data appendix, including the collecting procedure and data statistics. (NA)
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (NA)
    \item All datasets drawn from the existing literature (potentially including authors’ previously published work) are accompanied with appropriate citations. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available (yes)
    \item All datasets that are not publicly available are described in details. (NA)
    \item The preprocessing details of datasets are included. (NA)
    \item Details of Train/Valid/Test splits are included. (NA)
\end{itemize}








\subsection{Does this paper include novel models and algorithms? (yes)}

If yes, please complete the list below.

\begin{itemize}
    \item The input and output, mathematical setting, and algorithms are clearly introduced. (yes)
    \item The complexity analysis including time, space, and sample size is presented. (yes)
\end{itemize}


\subsection{Does this paper include computational experiments? (yes)}

If yes, please complete the list of experiment results below.

\begin{itemize}
    \item The evaluation metrics are formally described and the reasons for choosing these metrics are explained. (yes)
    \item Detailed hyperparameter settings of algorithms are described, including the ranges and how to select the best ones. (yes)
    \item The computing infrastructure for running experiments is described in detail, including GPU/CPU models, amount of memory, operating system. (yes)
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
    \item The number of training and inference runs are stated explicitly. (NA)
    \item Average training and inference time. (NA)
\end{itemize}


\subsection{Please also complete the list of source code below.}


\begin{itemize}
    \item All source code required for conducting experiments are uploaded as attachments (no). \\
    \textbf{Since the proprietary rights of the source code belong to a private company, the code cannot be published. However, the paper includes sufficient formulations, algorithms and measures to reproduce our experiments.}
    \item All source code required for conducting experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes (no) \\
    \textbf{Same as above.}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a clear way to allow replication of results. (yes) 
    \item The specification of dependencies is described, including the names and versions of relevant software libraries and frameworks. (yes)
    \item A README is provided to explain the structure of the source code, and how to obtain different results in the submission with corresponding scripts. (no) \\
    \textbf{Same as above.}
    \item The scripts or commands that are used to obtain results in different tables/figures are provided. (no) \\ 
    \textbf{Same as above.}
\end{itemize}
\end{comment}


\end{appendices}


==> poster.tex <==
\begin{itemize}
    \item Both riders 1\&2 want to go to B.
    \item Rider $i$ report “value of time” $\gamma_i$.
    \item Mechanism: allocation $\pi$ \& payment $x_i(\pi)$
    \item Rider cost: $c_i(\pi)$=travel time$*\gamma_i$
    \item Rider utility: $u_i(\pi)=-c_i(\pi)-x_i(\pi)$
    \item Discount price if rider 1 detours for pickup.
\end{itemize}

\begin{equation}
 \left.
 \begin{array}{ll}
 &\underset{\substack{(\pi,x)\in \Pi\times \mc{X}}}{\min}\sum_{i \in \mc{N}}c_i(\pi)+c_F(\pi)\\
 \\
 s.t.&
u_i(\pi)\ge-c_i^0,\\
\\
&\sum_{i \in \mc{N}}x_i(\pi)\ge c_F(\pi), \\
\\
&u_i(\pi(\gamma_i,\gamma_{-i}))\ge u_i(\pi(\gamma_i',\gamma_{-i})). 
%~\forall \gamma_i' \in \Gamma,  ~\forall i \in  \mc{N}, \forall \gamma_{-i} \in \Gamma^{N-1},
\\
\\
 \end{array}
 \right.
\end{equation}

Social optimum (SO): \\System tries to minimize rider cost $+$ fuel cost.

